Blocklength-Limited Performance of Relaying under Quasi-Static Rayleigh Channels

In this paper, the blocklength-limited performance of a relaying system is studied, where channels are assumed to experience quasi-static Rayleigh fading while at the same time only the average channel state information (CSI) is available at the source. Both the physical-layer performance (blocklength-limited throughput) and the link-layer performance (effective capacity) of the relaying system are investigated. We propose a simple system operation by introducing a factor based on which we weight the average CSI and let the source determine the coding rate accordingly. In particular, we prove that both the blocklength-limited throughput and the effective capacity are quasi-concave in the weight factor. Through numerical investigations, we show the appropriateness of our theoretical model. In addition, we observe that relaying is more efficient than direct transmission. Moreover, this performance advantage of relaying under the average CSI scenario is more significant than under the perfect CSI scenario. Finally, the speed of convergence (between the blocklength-limited performance and the performance in the Shannon capacity regime) in relaying system is faster in comparison to the direct transmission under both the average CSI scenario and the perfect CSI scenario.

==> 3_Overall_rate.tex <==

In~\eqref{eq:Overall_error_pro}, the relationship between the overall error probability and the error probability of single links is presented. From~\eqref{eq:single_link_error_pro}, the  error probability of a single link is subject to the related  raw rate . Therefore, in the following we further investigate the overall error probability by determining the overall  raw rate . 
As the channel information of all the three links are available at the source, the source is able to choose the  raw rate  which fulfills the channel conditions. 
As the  raw rate  of the two phases are the same, the source determines the  raw rate  of each frame 
based on the bottleneck link which is either the backhaul link or the combined link.
In other words, the  raw rate  is subject to  $\min \{{\bf{h}}_2^2, {\bf{h}}_1^2  + {\bf{h}}_3^2 \}$. 
%%Obviously, the overall error probability is subject to the channel qualities: ${\bf{h}}_1^2 $, ${\bf{h}}_2^2 $ and ${\bf{h}}_3^2 $. Firstly, ${\bf{h}}_1^2  + {\bf{h}}_3^2 $ determine the received SNR at the destination, it directly affects the decoding error probability at destination. Secondly, the relay cannot forward the data packet if error decoding happens at it,  which rapidly reduce the received SNR at the destination. In other words, ${\bf{h}}_2^2 $ affects the overall performance indirectly. %  Note that the raw  rate of all the three links should be the same.  
%Therefore, either  ${\bf{h}}_1^2  + {\bf{h}}_3^2 $ (directly) or ${\bf{h}}_2^2 $ is able to restrict the system performance. 
%
%Regarding the relationship  between $ {\bf{h}}_2^2$ and ${\bf{h}}_1^2  + {\bf{h}}_3^2$, 
We therefore investigate the overall error probability based on the following two cases:
\begin{itemize}
\item  {\bf{Case 1}}: ${\bf{h}}_2^2   \ge {\bf{h}}_1^2   + {\bf{h}}_3^2  $, which means the relay backhaul (source-relay) link is stronger than the combined link to the destination. If the target error probability of the combined link is set as ${{{\Pr}}}^{{\rm{e}}}_{\rm{co}}$, % from~\eqref{eq:single_link_data_rate} the  raw  rate of each phase $r$ can be determined based on the combined channel gain ${\bf{h}}_1^2 + {\bf{h}}_3^2 $. Hence,
 the overall  raw  rate decided by the source can be expressed as $r_{\rm{RA}}  = {\frac{1}{2}} r({\bf{h}}_1^2   + {\bf{h}}_3^2 , {{{\Pr}}}^{{\rm{e}}}_{\rm{co}},2m )$. Hence, the relative overall error probability is a function of  ${\Pr} _{{\rm{co}}}^{\rm{e}}$ and is obtained by:
\begin{equation}
\label{eq:error_pro1}
{\Pr} _{{\rm{RA}}}^{\rm{e}}({\Pr} _{{\rm{co}}}^{\rm{e}}) = {{\Pr} ^{\rm{e}}}\left( {{\bf{h}}_2^2,2{r_{{\rm{RA}}}},2m} \right) + \left( {1 - {{{\Pr} }^{\rm{e}}}\left( {{\bf{h}}_2^2,2{r_{{\rm{RA}}}},2m} \right)} \right) \cdot {\Pr} _{{\rm{co}}}^{\rm{e}} \mathrm{.}
 \end{equation}
Then ${{{\Pr}}}^{{\rm{e}}} [{\bf{h}}_2^2  ,r({\bf{h}}_1^2   + {\bf{h}}_3^2  , {{{\Pr}}}^{{\rm{e}}}_{\rm{co}} )] \le  {{{\Pr}}}^{{\rm{e}}}_{\rm{co}}$, hence we have:
\begin{equation}
\label{eq:upperboundOverall_error_pro1}
%{{{\Pr}}}_{\rm{co}}^{{\rm{e}}}\le 
{{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}  ( {{{\Pr}}}^{{\rm{e}}}_{\rm{co}} ) \le 
2{{{\Pr}}}_{{\rm{co}}}^{\rm{e}}  - \left( {{{{\Pr}}}_{{\rm{co}}}^{\rm{e}} } \right)^2 \mathrm{.}
\end{equation}
Especially, ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}} \! ( {{{\Pr}}}^{{\rm{e}}}_{\rm{co}} )\! \approx \!  {{{\Pr}}}^{{\rm{e}}}_{\rm{co}} $ when ${\bf{h}}_2^2   \gg   {\bf{h}}_1^2   + {\bf{h}}_3^2 $.
\item {\bf{Case 2}}:  ${\bf{h}}_2^2   < {\bf{h}}_1^2   + {\bf{h}}_3^2  $, the bottleneck link is the backhaul link. % Hence, the overall  raw  rate can be determined based on the backhaul channel gain ${\bf{h}}_2^2 $ and the related target error probability ${{{\Pr}}}_2^{{\rm{e}}}$.
 In this case, $r_{\rm{RA}}  = {\frac{1}{2}} r({\bf{h}}_2^2  ,{{{\Pr}}}_2^{{\rm{e}}},2m )$ while the overall error probability is the function of ${{{\Pr}}}_2^{{\rm{e}}}$:
\begin{equation}
\label{eq:error_pro2}
\!{{{\Pr}}}^{{\rm{e}}} _{\rm{RA}} ({{{\Pr}}}_2^{{\rm{e}}}) \! =\! {{{\Pr}}}_2^{{\rm{e}}} + 
 \left( {1 \! -\! {{{\Pr}}}_2^{{\rm{e}}} } \right)\cdot {{{\Pr}}}^{{\rm{e}}} \left( {{\bf{h}}_1^2  \!+\! {\bf{h}}_3^2  ,r_{\rm{RA}},2m} \right) \mathrm{.}
\end{equation}

Similarly, the upper bound of ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}$ can be given by:
\begin{equation}
\label{eq:upperboundOverall_error_pro2}
%{{{\Pr}}}_2^{{\rm{e}}}\le
{{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}  ({{{\Pr}}}_2^{{\rm{e}}} ) \le
2{{{\Pr}}}_2^{\rm{e}}  - \left( {{{{\Pr}}}_2^{\rm{e}} } \right)^2 \mathrm{.}
\end{equation}
Especially, ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}} ({{{\Pr}}}_2^{{\rm{e}}} ) \approx {{{\Pr}}}_2^{{\rm{e}}} $ when $  {\bf{h}}_1^2   + {\bf{h}}_3^2  \gg {\bf{h}}_2^2  $.
\end{itemize}

%Firstly, the overall probability is  strongly subject to the error probability target of the bottleneck  link.
Section~\ref{sec:The_Effective_Rate} will show that by choosing an appropriate error probability target for the bottleneck link, the BL-capacity of the system is able to be maximized. 



Firstly, combining~\eqref{eq:upperboundOverall_error_pro1} and~\eqref{eq:upperboundOverall_error_pro2} with~\eqref{eq:LowerboundOverall_error_pro}, the overall error probability of relaying can be bounded by:
\begin{equation}
\label{eq:final_bounds}
2{{\Pr}}_j^{\rm{e}}  - \left( {{{\Pr}}_j^{\rm{e}} } \right)^2  \ge {{\Pr}}_{{\rm{RA}}}^{\rm{e}}  \ge {{\Pr}}_j^{\rm{e}} \; \mathrm{,}
\end{equation}
where ${\Pr} _j^{\rm{e}}  = \max \{ {{\Pr}}_{{\rm{co}}}^{\rm{e}} ,{\Pr} _2^{\rm{e}} \} $ is the error probability of the bottleneck link:  ${{{\Pr}}}^{{\rm{e}}} _j= {{{\Pr}}}^{{\rm{e}}} _{\rm{co}}$ if $ {\bf{h}}_2^2   \ge {\bf{h}}_1^2   + {\bf{h}}_3^2 $ and  ${{{\Pr}}}^{{\rm{e}}} _j= {{{\Pr}}}^{{\rm{e}}} _{2}$ if $ {\bf{h}}_2^2   <{\bf{h}}_1^2   + {\bf{h}}_3^2 $.
%\begin{equation}
% {{{\Pr}}}^{{\rm{e}}} _j= \left\{ { \begin{array}{*{20}c}
 %  {{{\Pr}}}^{{\rm{e}}} _{\rm{co}} & {if \; {\bf{h}}_2^2   \ge {\bf{h}}_1^2   + {\bf{h}}_3^2  }  \\
  % {{{\Pr}}}^{{\rm{e}}} _2 & {if \; {\bf{h}}_2^2   < {\bf{h}}_1^2   + {\bf{h}}_3^2  }  \\
%\end{array}} \right. \; \mathrm{.}
%\end{equation}




Secondly, the overall  raw rate  can be given based on the function of~\eqref{eq:single_link_data_rate} by: 
\begin{equation}
\label{eq:overalldatarate}
% r_{\rm{RA}}= \left\{ { \begin{array}{*{20}c}
%   {\frac{1}{2}} r({\bf{h}}_1^2   + {\bf{h}}_3^2 , {{{\Pr}}}^{{\rm{e}}}_{\rm{co}} ) & {if \; {\bf{h}}_2^2   \ge {\bf{h}}_1^2   + {\bf{h}}_3^2  }  \\
%   {\frac{1}{2}} r({\bf{h}}_2^2  ,{{{\Pr}}}_2^{{\rm{e}}} ) & {if \; {\bf{h}}_2^2   < {\bf{h}}_1^2   + {\bf{h}}_3^2  }  \\
%\end{array}} \right.
r_{{\rm{RA}}}  = 0.5 r\left( {\min \left\{ {{\bf{h}}_2^2 ,{\bf{h}}_1^2  + {\bf{h}}_3^2 } \right\}, \max \left\{ {{\Pr} _2^{\rm{e}} ,{\Pr} _{{\rm{co}}}^{\rm{e}} } \right\}}, 2m \right)\mathrm{.}
\end{equation}

%Obviously, for fixed channel conditions, the overall  raw rate  is totally subject to the error probability of the bottleneck link.
Thirdly,~\eqref{eq:error_pro1} and~\eqref{eq:error_pro2} show that the overall error probability ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}$ is fully determined by the overall  raw rate  $r _{\rm{RA}}$. 
It is also shown in~\eqref{eq:overalldatarate} that for fixed channel conditions $r _{\rm{RA}}$ is further totally subject to the error probability of the bottleneck link ${{{\Pr}}}^{{\rm{e}}} _j$.
As a result, ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}$ is completely subject to ${{{\Pr}}}^{{\rm{e}}} _j$.
In other words, with non-fading channels the system is able to achieve the target overall error probability by choosing an appropriate  value of ${{{\Pr}}}^{{\rm{e}}} _j$.
In fact, ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}({{{\Pr}}}^{{\rm{e}}} _j)$ has the following characteristic:
%The relationship between them are presented in the Proposition 2.
%
%Then, for a target overall error probability $\hat{{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}$, the overall maximal achievable rate can be modeled as the follow problem: 
%\begin{equation}
%\begin{array}{l}
% \mathop {\max } \limits_{{{{\Pr}}}^{{\rm{e}}} _j } {r_{\rm{RA}} ({{{\Pr}}}^{{\rm{e}}} _j) } \\ 
% s.t.: \; {{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}  \left( {{{{\Pr}}}^{{\rm{e}}} _j } \right) \le \hat {{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}   \\ 
% \end{array} \; \mathrm{.}
%\end{equation}
%
%Obviously, $r_{\rm{RA}} $ is an increasing function in ${{{\Pr}}}^{{\rm{e}}} _j$, hence the solution to the above problem is equivalent to the solution to the follow problem: 
%\begin{equation}
%\begin{array}{l}
% \mathop {\max }{{{{\Pr}}}^{{\rm{e}}} _j }  \\ 
% s.t.: \; {{{\Pr}}}^{{\rm{e}}} _{\rm{RA}} \left( {{{{\Pr}}}^{{\rm{e}}}_j } \right) \le \hat{{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}  \\ 
% \end{array} \; \mathrm{.}
%\end{equation}
%\newtheorem{theorem2}{Proposition}
%\begin{theorem2}
%if the $ {\rm{ }}\frac{{xP_{{\rm{tx}}} }}{{\sigma ^2 }} > 0$~$dB$ $\forall$ $x={\bf{h}}_1^2 $, ${\bf{h}}_2^2 $ and ${\bf{h}}_3^2 $,   $\varepsilon _{\rm{O}} (\varepsilon _i )$ is increasing in $\varepsilon _i$.
%\label{th:monn-dec2}
%\end{theorem2}
\

\noindent
\textbf {Proposition 2 } \emph {The overall error probability ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}  ({{{\Pr}}}^{{\rm{e}}} _j )$ is strictly increasing in ${{{\Pr}}}^{{\rm{e}}} _j$. }


We provide here the proof under the assumption that ${\bf{h}}_2^2   \ge {\bf{h}}_1^2   + {\bf{h}}_3^2 $, the other situation can be proved similarly.
\begin{proof}
$\because$  ${\bf{h}}_2^2   \ge {\bf{h}}_1^2   + {\bf{h}}_3^2 $% , the overall probability is given by 

$\therefore$ ${{\Pr}}_{{\rm{RA}}}^{\rm{e}}({{{\Pr}}}_{{\rm{co}}}^{\rm{e}} )  = {{\Pr}}^{\rm{e}} [{\bf{h}}_2^2 ,r({\bf{h}}_1^2  + {\bf{h}}_3^2 ,{{\Pr}}_{{\rm{co}}}^{\rm{e}},2m )] + \left( {1 - {{\Pr}}^{\rm{e}} [{\bf{h}}_2^2 ,r({\bf{h}}_1^2  + {\bf{h}}_3^2 ,{{\Pr}}_{{\rm{co}}}^{\rm{e}},2m )]} \right)\cdot {{\Pr}}_{{\rm{co}}}^{\rm{e}} $.




$\therefore$ the derivative of ${{\Pr}}_{\rm{RA}}^{\rm{e}}$ with respect to ${{\Pr}}_{\rm{co}}^{\rm{e}}$ can be obtained by:
%
\begin{equation}
\label{eq:derivativesOverallPr_co}
  \frac{{\partial {{\Pr}}_{{\rm{RA}}}^{\rm{e}} ({{{\Pr}}}_{{\rm{co}}}^{\rm{e}} )}}{{\partial {{{\Pr}}}_{{\rm{co}}}^{\rm{e}} }}= \frac{{\partial {{{\Pr}}}_{{}}^{\rm{e}} ({{{\Pr}}}_{{\rm{co}}}^{\rm{e}} )}}{{\partial r}}\frac{{\partial r}}{{\partial {{{\Pr}}}_{{\rm{co}}}^{\rm{e}} }} 
=\left[ {\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{}} }}\left( {1 - {{\Pr}}_2^{\rm{e}} } \right) + \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{}} }}\left( {1 - {{\Pr}}_{{\rm{co}}}^{\rm{e}} } \right)} \right]\frac{{\partial r}}{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }} \; \mathrm{.}
\end{equation}


$\because$ $r({\bf{h}}_1^2   + {\bf{h}}_3^2  , {{{\Pr}}}^{{\rm{e}}}_{{\rm{co}}},2m )$ is the increasing in $ {{{\Pr}}}^{{\rm{e}}}_{{\rm{co}}}$ as well as ${{{\Pr}}}^{{\rm{e}}} (x, r, 2m)$ is increasing in $ r$,

$\therefore$ $\frac{{\partial {{{\Pr}}}_1^{\rm{e}} }}{{\partial r}} > 0$, $\frac{{\partial {{{\Pr}}}_2^{\rm{e}} }}{{\partial r}} > 0$ and $\frac{{\partial r}}{{\partial {{{\Pr}}}_{{\rm{co}}}^{\rm{e}} }}> 0$.

%$\because$ ${\bf{h}}_1^2   + {\bf{h}}_3^2 \ge {\bf{h}}_1^2$,

%$\therefore$ ${{\rm{Pr}}_1^{\rm{e}}  \ge {\rm{Pr}}_{{\rm{co}}}^{\rm{e}} }$.
 
$\because$ $0 \le {\rm{Pr}}_2^{\rm{e}}  \le 1$ and $0 \le {\rm{Pr}}_{\rm{co}}^{\rm{e}}  \le 1$

$\therefore$ based on~\eqref{eq:derivativesOverallPr_co}, ${{\partial \Pr _{{\rm{RA}}}^{\rm{e}} (\Pr _{{\rm{co}}}^{\rm{e}} )} \mathord{\left/
 {\vphantom {{\partial \Pr _{{\rm{RA}}}^{\rm{e}} (\Pr _{{\rm{co}}}^{\rm{e}} )} {\partial \Pr _{{\rm{co}}}^{\rm{e}} }}} \right.
 \kern-\nulldelimiterspace} {\partial \Pr _{{\rm{co}}}^{\rm{e}} }} > 0$.

$\therefore$ ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}  ({{{\Pr}}}^{{\rm{e}}} _{{\rm{co}}} )$ is strictly increasing in ${{{\Pr}}}^{{\rm{e}}} _{{\rm{co}}}$.
\end{proof}

So far, the overall  raw rate  and the overall error probability have been investigated for the relay system  with non-fading channels. Based on this, we  study the BL-capacity of the relay system under the finite blocklength regime.
%


\subsection{The BL-capacity}
\label{sec:The_Effective_Rate}

Based on~\eqref{eq:single_link_data_rate}, the raw rate of each phase $r$ is increasing in ${{{\Pr}}}^{{\rm{e}}} _j$. Therefore,  $r_{\rm{RA}}$ is also increasing in ${{{\Pr}}}^{{\rm{e}}} _j$ since $r_{\rm{RA}}=r/2$.
%Therefore, both the overall maximal rate $r_{\rm{RA}}$  and the overall error probability ${{{\Pr}}}^{{\rm{e}}}_{\rm{RA}}$ are increasing in ${{{\Pr}}}^{{\rm{e}}}_j$ the error probability of bottleneck link. 
Hence, the overall  raw rate  $r_{\rm{RA}}$  tends to infinity as long as ${{{\Pr}}}^{{\rm{e}}} _j$ goes to $1$. At the same time, the overall error probability also tends to 1. Note that the overall    raw rate  is not a successfully received/decoded data rate but a data rate based on the pure physical attempt to transmit bits from the source. So the destination decodes nothing correctly if the overall error probability is~1. Therefore, in order to investigate the effective performance of the relay system, it is more~meaningful to consider the correctly received data rate -- the BL-capacity. 
 % where the overall error probability is higher than 0.5. 

The service process $s_i$ of frame~$i$ (in bits per m channel use) is given based on the overall  raw rate :
\begin{equation}
s_i  = 2m \varphi r_{\rm{RA}}.
\end{equation}
where $\varphi$ is a binary random variable defined by  ${\Pr} \{ \varphi  = 1\}  = {1 - {{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}  }$ and ${\Pr} \{ \varphi  = 0\}  = { {{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}}$.
% 
Therefore, the BL-capacity, which is the expected value of the service process $s_i$,  is given by:
\begin{equation}
{\rm{E}}\left[ {s_i } \right] =  2\left( {1 -  {{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}  } \right)m \cdot  r_{\rm{RA}}\mathrm{.}
\label{eq:mean}
\end{equation}
We then have the following proposition on the BL-capacity:

%\

\noindent
\textbf {Proposition 3 } \emph {The BL-capacity ${\rm{E}}\left[ {s_i } \right]$ is a concave function in the overall  raw rate  $r_{\rm{RA}}$.}

Here we provide the proof under the situation that the bottleneck link is the backaul link, the other situation can be analyzed similarly. In addition, 
to simplify the proof of the proposition, we do not consider the extreme error situation.









%Therefore, the long expression of $\frac{{\partial {\rm{E}}\left[ {s_i } \right]}}{{\partial r_{{\rm{RA}}} }}$ can be divided into two parts:
%\begin{equation}
%\frac{{\partial {\rm{E}}\left[ {s_i } \right]}}{{\partial r_{{\rm{RA}}} }}={\mathop{\rm f}\nolimits} _{{\rm{In}}} \left( {r_{{\rm{RA}}} } \right) + {\mathop{\rm f}\nolimits} _{{\rm{De}}} \left( {r_{{\rm{RA}}} } \right)
%\end{equation}
%where ${\mathop{\rm f}\nolimits} _{{\rm{In}}} \left( {r_{{\rm{RA}}} } \right) $  and ${\mathop{\rm f}\nolimits} _{{\rm{De}}} \left( {r_{{\rm{RA}}} } \right)$ are the increasing part and decreasing part of the $\frac{{\partial {\rm{E}}\left[ {s_i } \right]}}{{\partial r_{{\rm{RA}}} }}$:
%\begin{equation}
%{\mathop{\rm f}\nolimits} _{{\rm{In}}} \left( {r_{{\rm{RA}}} } \right) = mr_{{\rm{RA}}} {{\Pr}}_{{\rm{co}}}^{\rm{e}} \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + mr_{{\rm{RA}}} \frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} {{\Pr}}_2^{\rm{e}} 
%\end{equation}
%\begin{equation}
%{\mathop{\rm f}\nolimits} _{{\rm{De}}} \left( {r_{{\rm{RA}}} } \right) = \left( {1 - {{\Pr}}_{{\rm{RA}}}^{\rm{e}} } \right)m - mr_{{\rm{RA}}} \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} - mr_{{\rm{RA}}} \frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}
%\end{equation}
%Then we get the relative derivatives of two parts with respective to $r_{\rm{RA}}$: 
%\begin{equation}
%\begin{array}{l}
% \frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{In}}} }}{{\partial r_{{\rm{RA}}} }} = m{\Pr} _{{\rm{co}}}^{\rm{e}} \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + m\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}{\Pr} _2^{\rm{e}}  \\ 
%  + mr_{{\rm{RA}}} \left( {2\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + {{\Pr}}_{{\rm{co}}}^{\rm{e}} \frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} + {{\Pr}}_2^{\rm{e}} \frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}} \right) \\ 
% \end{array}
%\end{equation}

%\begin{equation}
%\begin{array}{l}
% \frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{De}}} }}{{\partial r_{{\rm{RA}}} }} =  - 2m\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} - 2m\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + m{\Pr} _{{\rm{co}}}^{\rm{e}} \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + m{\Pr} _2^{\rm{e}} \frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} \\ 
 % - mr_{{\rm{RA}}} \left( {\frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} + \frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}} \right) \\ 
 %\end{array}
%\end{equation}

%Consider that 

%$\mathop {\lim }\limits_{r_{{\rm{RA}}}  \to 0} \frac{{\partial {\rm{E}}\left[ {s_i } \right]}}{{\partial r_{{\rm{RA}}} }} = m > 0$, therefore the following proposition holds if $\frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{In}}} }}{{\partial r_{{\rm{RA}}} }} < - {\frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{De}}} }}{{\partial r_{{\rm{RA}}} }}}$ where $r_{\rm{RA}}\in (0, \mathop {\min }\limits_{x_j  \in \left\{ {z_2 ,z_{co} } \right\}} \left\{ {\frac{1}{2}c\left( {x_j } \right)} \right\})$.

%\noindent
%\textbf {Proposition 3 } \emph {The mean of service rate ${\rm{E}}\left[ {s_i } \right]$ is a convex function of the overall  raw rate  $r_{\rm{RA}}$, $r_{\rm{RA}}\in (0, \mathop {\min }\limits_{x_j  \in \left\{ {z_2 ,z_{co} } \right\}} \left\{ {\frac{1}{2}c\left( {x_j } \right)} \right\})$.}




%\begin{proof}

%\noindent

%$\because$ ..XXXXXXXXXXXXXXXXXXXXXX


%$\therefore$  $-\frac{{\partial^2 {\mathop{\rm f}\nolimits} _{{\rm{De}}} }}{{\partial^2 r_{{\rm{RA}}} }} \ge  \frac{{\partial^2 {\mathop{\rm f}\nolimits} _{{\rm{In}}} }}{{\partial^2 r_{{\rm{RA}}} }}$

%$\because$ $\begin{array}{l}
%\mathop {\lim }\limits_{r_{{\rm{RA}}}  \to 0} \frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{In}}} }}{{\partial r_{{\rm{RA}}} }} = \mathop {\lim }\limits_{r_{{\rm{RA}}}  \to 0} - \frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{De}}} }}{{\partial r_{{\rm{RA}}} }} \\
%= m\left( {\mathop {\lim }\limits_{r_{{\rm{RA}}}  \to 0} \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + \mathop {\lim }\limits_{r_{{\rm{RA}}}  \to 0} \frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}} \right)\\
%\end{array}$

%$\therefore$  $\frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{In}}} }}{{\partial r_{{\rm{RA}}} }} < - {\frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{De}}} }}{{\partial r_{{\rm{RA}}} }}}$ when $r_{\rm{RA}}\in (0, \mathop {\min }\limits_{x_j  \in \left\{ {z_2 ,z_{co} } \right\}} \left\{ {\frac{1}{2}c\left( {x_j } \right)} \right\})$.  
%
%\end{proof}



%%%%%%%%%%%%%%%%%%%%%%proof%%%%%%%%%%%%end%%%%%%%%%%%%%%%%%%%%%%

%${\rm{3}}\frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + {\rm{3}}\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}\frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} \le \frac{{\partial ^{\rm{3}} {{\Pr}}_2^{\rm{e}} }}{{\partial ^{\rm{3}} r_{{\rm{RA}}} }}\frac{{\partial ^{\rm{3}} {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^{\rm{3}} r_{{\rm{RA}}} }}$

%So we have $2\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + {{\Pr}}_{{\rm{co}}}^{\rm{e}} \frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} + {{\Pr}}_2^{\rm{e}} \frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} > \frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} - \frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}$

%Hence$\frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{In}}} }}{{\partial r_{{\rm{RA}}} }} > \left| {\frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{De}}} }}{{\partial r_{{\rm{RA}}} }}} \right|$

%Hence we have the conclusion that: The mean of service rate ${\rm{E}}\left[ {s_i } \right]$ is first increasing and then decreasing in  $r_{{\rm{RA}}}$. 

Note that the overall  raw rate  $r_{{\rm{RA}}}$ is increasing in the overall error probability ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}$ and that the overall error probability ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}$ is increasing in the error probability  of the bottleneck link ${{{\Pr}}}^{{\rm{e}}} _i$, 
 we therefore have the following Proposition:

\noindent
\textbf {Proposition 4 } \emph {The BL-capacity ${\rm{E}}\left[ {s_i } \right]$ is first increasing and then decreasing in ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}$ or ${{{\Pr}}}^{{\rm{e}}} _i$. Thus, ${\rm{E}}\left[ {s_i } \right]$ has a unique maximum value.}
%

\
Proposition 4 shows that the BL-capacity of relaying is able to be maximized by choosing a proper target of ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}$ or ${{{\Pr}}}^{{\rm{e}}} _i$.


%\begin{equation}
%\frac{{\partial ^2 {\rm{E}}\left[ {s_i } \right]}}{{\partial ^2 r_{{\rm{RA}}} }} =  -
%2m\frac{{\partial {{\Pr}}_{{\rm{RA}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} - \frac{{\partial ^2 {{\Pr}}_{{\rm{RA}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}mr_{{\rm{RA}}} 
%\end{equation}





%\begin{equation}
%\begin{split}
% \frac{{\partial ^2 {{\Pr}}_{{\rm{RA}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} &= \frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}\left( {1 - {{\Pr}}_2^{\rm{e}} } \right) + \frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}\left( {1 - {{\Pr}}_{{\rm{co}}}^{\rm{e}} } \right) \\ 
%  &- 2\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} \\ 
% \end{split}
%\end{equation}


%We can learn that form Equation~\ref{eq:single_link_error_pro}:
%
%\begin{equation}
%\label{eq:single_link_error_derivative}
%\frac{{\partial {{\Pr}}_j^e }}{{\partial r}} = \sqrt {\frac{{2\pi m}}{{\left( {1 - 2^{ - 2c(x_j )} } \right)}}}  \cdot \frac{{e^{ - \frac{{m\left( {c(x_j ) - r} \right)^2 }}{{2\left( {1 - 2^{ - 2c(x_j )} } \right)\left( {\log _2 e} \right)^2 }}} }}{{\log _2 e}} > 0  \mathrm{,}
%\end{equation}
%
%\begin{equation}
%\label{eq:single_link_error_2derivative}
%\frac{{\partial ^2 {{\Pr}}_j^e }}{{\partial ^2 r}} = \frac{{m^{\frac{3}{2}} \sqrt {2\pi } \left( {c(x_j ) - r} \right)e^{ - \frac{{m\left( {c(x_j ) - r} \right)^2 }}{{2\left( {1 - 2^{ - 2c(x_j )} } \right)\left( {\log _2 e} \right)^2 }}} }}{{\left( {1 - 2^{ - 2c(x_j )} } \right)^{\frac{3}{2}} \left( {\log _2 e} \right)^3 }} \mathrm{.}
%\end{equation}

%Since the source determines the  raw rate  $r$ based on the perfect channel information, hence  raw rate  $r$ is smaller than the Shannon capacity of channel.
%Hence both $\frac{{\partial {{\Pr}}_j^e }}{{\partial r}}$ and $\frac{{\partial ^2 {{\Pr}}_j^e }}{{\partial ^2 r}} $ are positive.

%Then we divide the $\frac{{\partial {\rm{E}}\left[ {s_i } \right]}}{{\partial r_{{\rm{RA}}} }}$ into two parts:
%\begin{equation}
%\frac{{\partial {\rm{E}}\left[ {s_i } \right]}}{{\partial r_{{\rm{RA}}} }}={\mathop{\rm f}\nolimits} _{{\rm{In}}} \left( {r_{{\rm{RA}}} } \right) + {\mathop{\rm f}\nolimits} _{{\rm{De}}} \left( {r_{{\rm{RA}}} } \right)
%\end{equation}
%where ${\mathop{\rm f}\nolimits} _{{\rm{In}}} \left( {r_{{\rm{RA}}} } \right) $  and ${\mathop{\rm f}\nolimits} _{{\rm{De}}} \left( {r_{{\rm{RA}}} } \right)$ are the increasing part and decreasing part of the $\frac{{\partial {\rm{E}}\left[ {s_i } \right]}}{{\partial r_{{\rm{RA}}} }}$:
%\begin{equation}
%{\mathop{\rm f}\nolimits} _{{\rm{In}}} \left( {r_{{\rm{RA}}} } \right) = mr_{{\rm{RA}}} {{\Pr}}_{{\rm{co}}}^{\rm{e}} \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + mr_{{\rm{RA}}} \frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} {{\Pr}}_2^{\rm{e}} 
%\end{equation}
%\begin{equation}
%{\mathop{\rm f}\nolimits} _{{\rm{De}}} \left( {r_{{\rm{RA}}} } \right) = \left( {1 - {{\Pr}}_{{\rm{RA}}}^{\rm{e}} } \right)m - mr_{{\rm{RA}}} \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} - mr_{{\rm{RA}}} \frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}
%\end{equation}

%\begin{equation}
%\begin{array}{l}
% \frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{In}}} }}{{\partial r_{{\rm{RA}}} }} = m{\Pr} _{{\rm{co}}}^{\rm{e}} \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + m\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}{\Pr} _2^{\rm{e}}  \\ 
%  + mr_{{\rm{RA}}} \left( {2\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + {{\Pr}}_{{\rm{co}}}^{\rm{e}} \frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} + {{\Pr}}_2^{\rm{e}} \frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}} \right) \\ 
% \end{array}
%\end{equation}

%\begin{equation}
%\begin{array}{l}
% \frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{De}}} }}{{\partial r_{{\rm{RA}}} }} =  - 2m\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} - 2m\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + m{\Pr} _{{\rm{co}}}^{\rm{e}} \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + m{\Pr} _2^{\rm{e}} \frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} \\ 
%  - mr_{{\rm{RA}}} \left( {\frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} - \frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}} \right) \\ 
% \end{array}
%\end{equation}

%Then the 

%$\left\{ {2\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}} \right\}_{r_{{\rm{RA}}}  \to 0}  = \left\{ {\left( {1 - {{\Pr}}_{{\rm{co}}}^{\rm{e}} } \right)\frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} - \left( {1 - {{\Pr}}_2^{\rm{e}} } \right)\frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}} \right\}_{r_{{\rm{RA}}}  \to 0} $

%and

%${\rm{3}}\frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + {\rm{3}}\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}\frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} \le \frac{{\partial ^{\rm{3}} {{\Pr}}_2^{\rm{e}} }}{{\partial ^{\rm{3}} r_{{\rm{RA}}} }}\frac{{\partial ^{\rm{3}} {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^{\rm{3}} r_{{\rm{RA}}} }}$

%So we have $2\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + {{\Pr}}_{{\rm{co}}}^{\rm{e}} \frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} + {{\Pr}}_2^{\rm{e}} \frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} > \frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} - \frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}$

%Hence$\frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{In}}} }}{{\partial r_{{\rm{RA}}} }} > \left| {\frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{De}}} }}{{\partial r_{{\rm{RA}}} }}} \right|$

%Hence we have the conclusion that: The mean of service rate ${\rm{E}}\left[ {s_i } \right]$ is first increasing and then decreasing in  $r_{{\rm{RA}}}$. Note that the $r_{{\rm{RA}}}$ is the increasing function of the target overall error probability, therefore we have the follow Proposition:

%\noindent
%\textbf {Proposition 4 } \emph {The mean of service rate ${\rm{E}}\left[ {s_i } \right]$ is first increasing and then decreasing in the overall error probability ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}$.}


% 我们需要证明 overall probability 是 单调递增函数

%The $ r({\bf{h}}_1^2   + {\bf{h}}_3^2  , {{{\Pr}}}^{{\rm{e}}}_3 )$ has the following properties:
%\begin{itemize}
%  \item  $ r({\bf{h}}_1^2   + {\bf{h}}_3^2  , {{{\Pr}}}^{{\rm{e}}}_3 )$
%\end{equation}


%$1 slot = 0.5ms = 1/2000 s$

% m $=$ 200 to 600 means the $T_f =$ 0.1s to 0.3s .

==> 4_MSDR.tex <==
%\section{The system performance for fading channel}
\section{The BL-capacity with Fading Channels}
\label{sec:Effective_Rate_Block_Fading}
%
%\begin{equation}
%s_i  = \left\{ {\begin{array}{*{20}c}
%   {m\bar r(\alpha _1  + {\rm{h}}_3^2  )} & {with\;prob.\;\left[ {1 - \varepsilon (\alpha _2 )} \right] \cdot \left[ {1 - \varepsilon (\alpha _1  + {\rm{h}}_3^2  )} \right]}   \\
%   {m\bar r(\alpha _1 )} & {with\;prob.\;\varepsilon (\alpha _2 )\left[ {1 - \varepsilon (\alpha _1 )} \right]}   \\
%   0 & { 
%{with\;prob.\left[ {1 - \varepsilon (\alpha _2 )} \right]\varepsilon (\alpha _1  + {\rm{h}}_3^2  ) + \varepsilon (\alpha _2 )\varepsilon (\alpha _1 )}}   \\
%\end{array}} \right.
%\end{equation}
In this section,  we extend the  results of Section~\ref{sec:Effective_Rate_relay} to block-fading channels where the channel gains remain constant within a frame (two phases) and vary from one frame to the next. In other words, the channels are fixed  within every single two-phases transmission of a packet. %Therefore, the analysis of relaying performance with non-fading channels are still valid in each single frame of block-fading channels.% of the fading channels. 


%\subsection{Maximize the expected value of BL-capacity per frame} 

As the CSI of all the links are available at the source, %Based on our analysis in Section~\ref{sec:Effective_Rate_relay},
 the source is required to determine the value of overall  raw rate  $ r_{\rm{RA}} $ to maximize  the BL-capacity (the expected value of the service process) in each  frame. 
%Therefore, with the block-fading channels the source is able to  maximize the expected value of BL-capacity for each frame.
 As a result, the overall  raw rate  is varying along with the channel fading from frame to frame and can be denoted by $r _{{\rm{RA}},i}$ where $i$ is the index of frames.  Therefore, the service process $s_i$ under a block-fading channel assumption can be modeled as (in bits per m channel use):
\begin{equation}
s_i  =2m\phi_i r _{{\rm{RA}},i}\mathrm{,}
\end{equation}
where $\phi_i  $ is a binary random variable defined by   $\Pr \{ \phi_i  = 1\}  = {1\! -\!  {{\Pr}}^{{\rm{e}}} _{{\rm{RA}},i}  }$, $\Pr \{ \phi_i  = 0\}  = { {{\Pr}}^{{\rm{e}}} _{{\rm{RA}},i}  }$ and $r_{{\rm{RA}},i}$ is chosen by maximizing the expected value of $s_i$ for frame $i$.
%
Finally, the BL-capacity  over frames therefore can be obtained by the sample mean of the service process: %\footnote{The equation  presented in~\eqref{eq:mean__} is the mean of the service process. , the derivation of it will be presented in our future work.}:
${\rm{E}}\left[ {{s_i}} \right] = \mathop {\lim }\limits_{I \to  + \infty } \frac{{\sum\nolimits_{i = 1}^I {\left( {1 - \Pr _{{\rm{RA}},i}^{\rm{e}}} \right) \cdot 2m{r_{{\rm{RA}},i}}} }}{I}$. % = 2m \iint {\left( {1 - \Pr _{{\rm{RA}},i}^{\rm{e}}} \right) \cdot {r_{{\rm{RA}},i}}}d{x_{\rm{co}}}d{x_2}$
%\begin{equation}
% {\mathop{\rm E} } \left[ {s_i } \right] = \sum\nolimits_{i = 1}^{ + \infty } {\left( {1 - {\Pr}_{{\rm{RA,}}i}^{\rm{e}} } \right) \cdot %2mr_{{\rm{RA},}i}} 
%\; \mathrm{.}
%\label{eq:mean__}
%\end{equation}
%where the ${{\mathop{\rm E}\limits_z} \left[ {s_i } \right]} $ the expected value of $s_i$ over channel fading while $z$ denotes channel gain variable.

%In addition, the variance of the service rate $s_i$ can be obtained by:
%\begin{equation}
%\begin{split}
% {\mathop{\rm Var}\nolimits} \left[ {s_i } \right] = &\sum\nolimits_{i = 1}^{ + \infty } { { {\Pr}_{{\rm{RA,}}i}^{\rm{e}} {\mathop{\rm E}\nolimits} \left[ {s_i } \right]^2 } }  \\ 
%  + &\sum\nolimits_{i = 1}^{ + \infty } { {\left( {1 - {\Pr}_{{\rm{RA,}}i}^{\rm{e}} } \right)\left( {2mr_{{\rm{RA,}}i}  - {\mathop{\rm E}\nolimits} \left[ {s_i } \right]} \right)^2 }}  \\ 
% \end{split}
%\end{equation}


%\input{fixed_error_probability}

%\begin{equation}
%\begin{array}{l}
% \left( {c_1  + c_2 \cdot Q^{ - 1} \left( {\Pr _j^{\rm{e}} } \right)} \right) \\
% \left\{ \begin{array}{l}
% {{\Pr}}_2^{\rm{e}} \left( {\frac{{\partial ^2 {{\Pr}}_1^{\rm{e}} }}{{\partial ^2 r}}\left( {\frac{{\partial r}}{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}} \right)^2  + \frac{{\partial {{\Pr}}_1^{\rm{e}} }}{{\partial {\rm{r}}}}\frac{{\partial ^2 r}}{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}} \right) \\ 
%  + \left\{ {2\frac{{\partial {{\Pr}}_1^{\rm{e}} }}{{\partial r}}\frac{{\partial r}}{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }} - {\rm{1}}} \right\}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r}}\frac{{\partial r}}{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }} \\ 
%  + \left\{ {{{\Pr}}_1^{\rm{e}}  - {{\Pr}}_{{\rm{co}}}^{\rm{e}}  - 1} \right\}\left( {\frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r}}\left( {\frac{{\partial r}}{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}} \right)^2  + \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r}}\frac{{\partial ^2 r}}{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}} \right) \\ 
% \end{array} \right\} \\ 
%  > c_2 \left\{ \begin{array}{l}
% \left( {1 - {\Pr}_{{\rm{RA}}}^{\rm{e}} } \right) \cdot 2\pi Q^{ - 1} \left( {\Pr _j^{\rm{e}} } \right)e^{\left( {Q^{ - 1} \left( {\Pr _j^{\rm{e}} } \right)} \right)^2 }  \\ 
% \left\{ {{{\Pr}}_1^{\rm{e}}  - {{\Pr}}_{{\rm{co}}}^{\rm{e}} } \right\}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r}}\frac{{\partial r}}{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }} \cdot 2\sqrt {2\pi } e^{\frac{{\left( {Q^{ - 1} \left( {\Pr _j^{\rm{e}} } \right)} \right)^2 }}{2}}  \\ 
% \left\{ {{{\Pr}}_2^{\rm{e}} \frac{{\partial {{\Pr}}_1^{\rm{e}} }}{{\partial r}}\frac{{\partial r}}{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }} + 1 - {{\Pr}}_2^{\rm{e}} } \right\}2\sqrt {2\pi } e^{\frac{{\left( {Q^{ - 1} \left( {\Pr _j^{\rm{e}} } \right)} \right)^2 }}{2}}  \\ 
% \end{array} \right\} \\ 
% \end{array}
%\end{equation}

%What we need to prove:
%\begin{equation}
%\begin{array}{l}
% \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r}}\left( {c_1  + c_2 Q^{ - 1} \left( {\Pr _j^{\rm{e}} } \right)} \right) + \sqrt {2\pi } {{\Pr}}_2^{\rm{e}} \left( {c_1  + c_2 Q^{ - 1} \left( {\Pr _j^{\rm{e}} } \right)} \right)e^{\frac{{\left( {Q^{ - 1} \left( {\Pr _{{\rm{co}}}^{\rm{e}} } \right)} \right)^2 }}{2}}  \\ 
% \left\{ \begin{array}{l}
% \left( {\frac{{\partial ^2 {{\Pr}}_1^{\rm{e}} }}{{\partial ^2 r}} - \left( {1 + {{\Pr}}_{{\rm{co}}}^{\rm{e}}  - {{\Pr}}_1^{\rm{e}} } \right)\frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r}}} \right)c_2  +  \\ 
% \left( {\frac{{\partial {{\Pr}}_1^{\rm{e}} }}{{\partial {\rm{r}}}} - \left( {1 + {{\Pr}}_{{\rm{co}}}^{\rm{e}}  - {{\Pr}}_1^{\rm{e}} } \right)\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r}}} \right)Q^{ - 1} \left( {\Pr _{{\rm{co}}}^{\rm{e}} } \right) \\ 
%  + 2c_2 \frac{{\partial {{\Pr}}_1^{\rm{e}} }}{{\partial r}}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r}} \\ 
% \end{array} \right\} \\ 
%  > \left\{ \begin{array}{l}
% \left( {1 - {\Pr}_{{\rm{RA}}}^{\rm{e}} } \right) \cdot \sqrt {2\pi } Q^{ - 1} \left( {\Pr _j^{\rm{e}} } \right)e^{\frac{{\left( {Q^{ - 1} \left( {\Pr _{{\rm{co}}}^{\rm{e}} } \right)} \right)^2 }}{2}}  \\ 
% 2\left\{ {{{\Pr}}_1^{\rm{e}}  - {{\Pr}}_{{\rm{co}}}^{\rm{e}} } \right\}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r}}\frac{{\partial r}}{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }} \\ 
% 2\left\{ {{{\Pr}}_2^{\rm{e}} \frac{{\partial {{\Pr}}_1^{\rm{e}} }}{{\partial r}}\frac{{\partial r}}{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }} + 1 - {{\Pr}}_2^{\rm{e}} } \right\} \\ 
% \end{array} \right\} \\ 
% \end{array}
%\end{equation}



%\begin{equation}
%\frac{{\partial {{\Pr}}_j^{\rm{e}} }}{{\partial r}} = \frac{1}{{\sqrt {2\pi } }}\exp \frac{m}{2}\frac{{\left[ {\log \left( {1 + \frac{{z_j p_{{\rm{tx}}} }}{{\sigma ^2 }}} \right) - r} \right]^2 }}{{\left( {1 - \left( {1 + \frac{{z_j p_{{\rm{tx}}} }}{{\sigma ^2 }}} \right)^{ - 2} } \right)\left( {\log _2 e} \right)^2 }}
%\end{equation}

%\begin{equation}
%\frac{{\partial ^2 {{\Pr}}_j^{\rm{e}} }}{{\partial ^2 r}} = \frac{m}{{2\sqrt {2\pi } }}\frac{{\left[ {r - \log \left( {1 + \frac{{z_j p_{{\rm{tx}}} }}{{\sigma ^2 }}} \right)} \right]e^{\frac{m}{2}\frac{{\left[ {\log \left( {1 + \frac{{z_j p_{{\rm{tx}}} }}{{\sigma ^2 }}} \right) - r} \right]^2 }}{{\left( {1 - \left( {1 + \frac{{z_j p_{{\rm{tx}}} }}{{\sigma ^2 }}} \right)^{ - 2} } \right)\left( {\log _2 e} \right)^2 }}} }}{{\left( {1 - \left( {1 + \frac{{z_j p_{{\rm{tx}}} }}{{\sigma ^2 }}} \right)^{ - 2} } \right)\left( {\log _2 e} \right)^2 }}
%\end{equation}

%As proved in~\cite{Gursoy_2011} the average transmission rate over a (one hop) single link is a  concave function of the error probability of this link. Hence, the average transmission rate of the bottleneck link is a concave function of its error probability. In addition, as analyzed in \textbf {Proposition 2}, ${\rm{\Pr}}_{{\rm{RA}}}^e$ is the a increasing function of  ${\rm{\Pr}}_{j}^e$. It also can be proved that $\frac{{1 - \hat {\rm{\Pr}}_{{\rm{RA}}}^e ({\rm{\Pr}} _j^e )}}{{1 - {\rm{\Pr}} _j^e }}$ is increasing in ${\rm{\Pr}} _j^e$.
 


%Therefore the ${\rm{E}}\left[ {s_i } \right]$ can be expressed the as a product of a increasing function $incr({\rm{\Pr}} _{j}^{e})$ and a concave function $conc({\rm{\Pr}} _{j}^{e})$:
%\begin{equation}
%\begin{split}
%{\mathop{\rm E}\nolimits} \left[ {s_i } \right] &= incr({\rm{\Pr}} _{j}^{e}) \cdot  conc({\rm{\Pr}} _{j}^{e}) \\
%&= \frac{{(1 - \hat {\rm{\Pr}}_{{\rm{RA}}}^e )}}{{(1 - {\rm{\Pr}} _j^e )}} \cdot m(1 - {\rm{\Pr}} _{j}^{e} ){\mathop{\rm E}\nolimits} \left[ {r_{{\rm{RA}}} } ({\rm{\Pr}} _{j}^{e})\right]\\
%\end{split}
%\end{equation}

%\begin{proof}
%\textbf {the proof has not been finished}

%$\because$ the follow reasons:
%\begin{itemize}
%\item $conc({\rm{\Pr}} _{j}^{e})$ is first increasing and then decreasing in ${\rm{\Pr}} _{j}^{e}$.
%\item $incr({\rm{\Pr}} _{j}^{e})$ is increasing in ${\rm{\Pr}} _{j}^{e}$.
%\item both  $conc({\rm{\Pr}} _{j}^{e})$ and $incr({\rm{\Pr}} _{j}^{e})$  are positive.
%\end{itemize}
%$\therefore$ we have the follow conclusion:
%\begin{itemize}
%\item if    $\left. {\frac{{\partial {\rm{E}}\left[ {s_i } \right]}}{{\partial {\rm{\Pr}} _j^e }}} \right|_{{\rm{\Pr}} _j^e  \to 1}  \ge 0$   then the  ${\rm{E}}\left[ {s_i } \right]$ is increasing in ${\Pr} _{j}^{e}$.
%\item if   $\left. {\frac{{\partial {\rm{E}}\left[ {s_i } \right]}}{{\partial {\rm{\Pr}} _j^e }}} \right|_{{\rm{\Pr}} _j^e  \to 1}  < 0$    then the  ${\rm{E}}\left[ {s_i } \right]$ is first increasing and then decreasing in ${\rm{\Pr}} _{j}^{e}$.
%\end{itemize}

%\end{proof}
%
%Hence, the MSDR of the system (per m channel use) can be given as:
%\begin{equation}
%\left. {R } \right|_{\left\{ {d,P_d } \right\}}  \approx \frac{{{m \bar r_O}\left( {1 - \varepsilon _{\rm{O}} } \right)}}{2}\left( {1 + \sqrt {1 + \frac{{2\varepsilon _{\rm{O}} \ln \left( {P_d } \right)}}{{d\left( {1 - \varepsilon _{\rm{O}} } \right)}}} } \right) \mathrm{,}
%\label{eqn:effective_rate_final}
%\end{equation}
%and the normalized MSDR in bits per channel use is given as:
%\begin{equation}
%\left. {\bar R} \right|_{\left\{ {d,P_d } \right\}}\! =\! \frac{{\left. R \right|_{\left\{ {d,P_d } \right\}} }}{m} \! \approx \! \frac{{{ \bar r_O}\left( {1 \!-\! \varepsilon _{\rm{O}} } \right)}}{2}\left( {1 \!+\! \sqrt {1 \!+\! \frac{{2\varepsilon _{\rm{O}} \ln \left( {P_d } \right)}}{{d\left( {1 \!-\! \varepsilon _{\rm{O}} } \right)}}} } \right) \mathrm{.}
%\label{eqn:effective_rate_final}
%\end{equation}
%\noindent
%\textbf {Proposition 4 (miss proof)} \emph {For a given QoS requirement pair $\{d, P_d\}$, the maximum sustainable data rate is first increasing and later decreasing on overall error probability~$\bar \varepsilon_{\rm{O}}$.}%, and also a convex function of the bottleneck link error probability $\varepsilon_i$.}
%








==> v 2.7_single_black/0_beginning.tex <==
\title{Blocklength-Limited Performance of Relaying under Quasi-Static Rayleigh Channels}

% author names and affiliations
% use a multiple column layout for up to three different
% affiliations

%\author{\IEEEauthorblockN{Yulin Hu, James Gross,  Anke Schmeink and Tong Wang}}


%\author{\IEEEauthorblockN{Yulin Hu \\ UMIC Research Centre \\RWTH Aachen University, Germany \\
%Email: $hu$@umic.rwth-aachen.de \and James Gross \\ UMIC Research Centre \\RWTH Aachen University, Germany \\
%Email: $gross$@umic.rwth-aachen.de \and Anke Schmeink and Tong Wang \\ UMIC Research Centre \\RWTH Aachen University, Germany \\ Email:
%\{$schmeink$|$tong.wang$\}@umic.rwthaachen.de }}


% make the title area
\maketitle


\begin{abstract}
In this paper, the blocklength-limited performance of a relaying system is studied, where  channels are assumed to experience  quasi-static Rayleigh fading while at the same time only the average channel state information (CSI) is available at the source. 
Both the physical-layer performance (blocklength-limited throughput) and the { {link}}-layer performance (effective capacity) of the relaying system are investigated.  
We propose a simple system operation by introducing a factor based on which we weight the average CSI and let the source determine the coding rate accordingly.
In particular, we prove that both the { {blocklength-limited throughput}} and the effective capacity  are quasi-concave in the weight factor. %In other words, the blocklength-limited  (either the physical-layer or the higher-layer) performance of the system can be easily optimized based on the proposed operation by choosing an appropriate weight factor.
%Moreover, we prove that the BL-capacity is strictly increasing in blocklength while the effective capacity is concave in the blocklength. Hence the blocklength is also an important factor in the design of QoS-support relaying systems.
Through numerical investigations, we show the appropriateness of our theoretical model. { {In addition, we observe that relaying is more efficient than direct transmission. Moreover,  this performance advantage of relaying under the average CSI scenario is more significant than under the perfect CSI scenario. Finally, the speed of convergence (between the blocklength-limited performance and the performance in the Shannon capacity regime) in relaying system is faster in comparison to the direct transmission under both the average CSI scenario and the perfect CSI scenario.}}
%Moreover, we evaluate the performance of the studied relaying system (with average CSI) in comparison to  either relaying with perfect CSI or direct transmission.
\end{abstract}
%
\begin{keywords}
Finite blocklength, decode-and-forward, relaying, throughput, effective capacity, average CSI.
\end{keywords}



%\section*{Acknowledgment}
%This work is supported by


==> v 2.7_single_black/1_Introduction.tex <==
\section{Introduction}
\label{sec:Introduction}
%Future wireless communication networks are expected to support high traffic while providing quality of service (QoS) guarantees, e.g., queuing delays and delay violation probabilities. 
%By taking the statistical QoS provisioning into account, Wu and Negi~\cite{Dapeng_2003} proposed the effective capacity which is a function combining physical-layer performance and queuing performance. More precisely, for given QoS constraints, the maximum arrival rate that the system can sustain is subject to the effective capacity.   
%Hence, the effective capacity and the effective-capacity-based performances essentially provide suitable metrics for QoS-constrained services and can be used for the design of QoS-support systems.

%Cooperative communications can achieve spatial diversity and multiplexing without requiring multiple-antennas to be  collocated in a single device. The three-terminal relay channel, as the fundamental unit of cooperative communications, was introduced in the pioneering work [6] and thoroughly analyzed in [7]. Although early information theoretic studies on cooperative communications focussed on full-duplex relaying, in recent years a lot of research has been directed towards practical protocols based on half-duplex relaying, where the relay is not able to receive and transmit simultaneously, e.g. [1]–[4], [8]. Among the various strategies that enable relays to assist the source-to-destination communication link, the decode-and-forward (DF) strategy has attracted great attention. In DF, the transmission interval is divided into a listening phase, during which a relay only receives, and a collaboration phase, during which the relay transmits the successfully decoded source message. The duration of the listening phase can be predetermined [3], [4] or it can be adapted to the actual quality of the source-to-relay channel [8]–[11]. In case of the latter, and in the absence of channel state information (CSI) at the sender, the relay would decide on its own when to switch from listening to collaborating, which is also referred to as dynamic decode-and-forward (DDF) [10]. 


In wireless communications, relaying~\cite{Laneman_2004,  Karmakar_2011, Yuzhen_2014} is 
well known as an efficient way to mitigate wireless fading by exploiting spatial diversity.  
Specifically, two-hop decode-and-forward (DF) relaying protocols significantly improve the capacity
and quality of service~\cite{Wendong_2011, Yulin_2011,My_WD2012_effective_capacity,Bhatnagar_2013}.  
{However, all the above studies of the advantages of relaying are under the ideal assumption of communicating arbitrarily reliably at Shannon's channel capacity, i.e.,  coding is assumed to be performed using a block with an infinite length.}% 



{{In the finite blocklength regime, especially when the blocklength is short, the error probability of the communication becomes no longer negligible.}} Recently, an accurate approximation of achievable coding rate is  identified in [8,~Thm.~54] for a single-hop transmission system while taking the error probability into account.  
In~\cite{Verdu_2010} the authors show that the performance loss due to a finite blocklength is considerable and becomes more significant when the blocklength is relatively short.  {{Moreover,   this fundamental study regarding AWGN channels has been extended to Gilbert-Elliott Channels~\cite{Polyanskiy_2011}, quasi-static fading channels~\cite{Yang_2014},~\cite{Gursoy_2013}, quasi-static fading channels with retransmissions~\cite{Peng_2011,Makki_2014} as well as  spectrum sharing networks~\cite{Makki_2015}.  However, all these works focus on single-hop non-relaying systems while the study of the blocklengh-limited performance of relaying is missing.}}


In a two-hop relaying network, relaying exploits spatial diversity but at the same time halves the blocklength of the transmission (if equal time division is considered). 
As has been shown in~\cite{Verdu_2010}  that the performance loss due to a finite blocklength is considerable and becomes more significant when the blocklength is relatively short,  the relaying performance  {in}  the finite blocklength regime becomes interesting.
In our recent work~\cite{Hu_2015}, we address  in general analytical performance
models for relaying with finite blocklengths. We investigate the blocklength-limited throughput (BL-throughput) of relaying, {{where the BL-throughput is %a    performance metric (like the outage capacity) for transmissions with errors and 
defined by  the average of correctly decoded bits at the destination per channel use.}
%Moreover, we prove that the BL-throughput of relaying is quasi-concave in the overall error probability of relaying.
{{{We observe by simulations in~\cite{Hu_2015}  that the performance loss (due to a finite blocklength) of relaying is much smaller than expected, while the performance loss of direct transmission is larger. This observation shows the performance advantage of relaying  {in}  the  finite blocklength regime (in comparison to direct transmission).}}}  %seems counterintuitive as relaying halves the blocklength.
    {{{We further show the reason of this performance advantage in~\cite{Hu_letter_2015} that  relaying has a higher SNR at each hop (in comparison to direct transmission) which makes it set the coding rate more aggressively.}}}%, this results in a higher BL-throughput.}}}


Our previous work in either~\cite{Hu_2015} or~\cite{Hu_letter_2015} is under static channels and with an assumption that {{{the source has perfect channel state information (CSI) of all the links}}}.   %Under this perfect CSI assumption, the  transmission errors are purely due to the noise (which may make the code be not able to be averaged). 
In this paper, we generalize the work in~\cite{Hu_2015} and~\cite{Hu_letter_2015}
 into a scenario with quasi-static Rayleigh channels. 
Under the quasi-static fading model, channels vary from one transmission period to the next. Unlike the static channel model, it may be too optimistic  in practice to have instantaneously perfect CSI of all the fading channels (of the relaying system) {{{at the source}}}. However, if the source does not have perfect CSI, e.g., only the average CSI is available at the source, it is not able to determine an appropriate coding rate to fit the instantaneous channel. %Therefore, it is likely that the coding rate set by the source based on the average CSI is higher than the Shannon capacity of the instantaneous channel. {{According to~\cite{Verdu_2010}, this (coding rate is higher than the Shannon capacity) results in a significant error probability which is higher than 0.5.}}   
Thus, the  analysis and improvement of the blocklength-limited performance of such a relaying system (under quasi-static fading channels but  only with average CSI) becomes interesting and also challenging. To the best of our knowledge, these issues have not been studied in detail so far.  


Under the described relaying system (with quasi-static fading channels and average CSI), 
%In this work,  we focus on the blocklength-limited performance of the above relaying system, where quasi-static fading channels are considered while  only the average CSI is assumed to be available at the source.  
%Under the described system, 
 we investigate both the physical-layer performance, e.g., BL-throughput, and the  {{link}-layer performance, e.g., effective capacity\footnote{{{The effective capacity  is a famous performance model that accounts for transmission and queuing effects~\cite{Dapeng_2003}. It characterizes the (maximum) arrival rate of a flow to a queuing system and
relates the stochastic characterization of the service of the queuing system to a queue-length or delay constraints
of the flow. It has been widely applied to the analysis of wireless systems~\cite{Ren_2009,Harsini_2012,Gursoy_2013}. However, no effective capacity analysis
of relaying under finite blocklength model has been published so far to the best of our knowledge.}}}.
We propose a simple system operation by introducing a factor based on which we weight the average CSI and let the source determine the coding rate accordingly.
In particular, we prove that both the  BL-throughput and the effective capacity  are quasi-concave in the weight factor. % In other words, the performance can be easily optimized based on the proposed operation.
%
By simulations, we show the  appropriateness of our theoretical model. In addition, we show that  the BL-throughput of relaying is slightly increasing in the blocklength while the effective capacity is significantly decreasing in the blocklength. %This is an important guideline for the design of a QoS-support system.  
Moreover, we %evaluate the performance of the studied relaying system (with average CSI) in comparison to  relaying with perfect CSI and non-relaying transmission. We 
observe  the performance advantage of relaying  {in}  the  finite blocklength regime:  Under the condition of having similar Shannon capacity performance,  relaying outperforms direct transmission in the finite blocklength regime.
More importantly, this performance advantage  under the average CSI scenario is more significant than under the perfect CSI scenario.  Finally, we find that the performance loss due to a finite blocklength (the gap between BL-throughput and Shannon/outage capacity) is negligible under the average CSI scenario in comparison to under the perfect CSI scenario.







The rest of the paper is organized as follows. Section~\ref{sec:Preliminaries} describes the system model and briefly introduces the background theory regarding the finite blocklength regime. 
In Section~\ref{sec:Physical_layer_P}, we consider the physical-layer performance and derive the BL-throughput of the relaying system. Subsequently, in  Section~\ref{sec:Higher_layer_P} the link-layer performance of the relaying system is studied, where the distribution of the service process increment and the maximum sustainable date rate are investigated.  
Section~\ref{sec:simulation} presents our simulation results. % and shows the relay performance with finite blocklength. 
Finally, we conclude our work in Section~\ref{sec:Conclusion}.


%Regarding the notation,  notation $E(\bf{A})$ and
%$Tr(\bf{A})$ denote the expectation and trace operation of matrix
%$\bf{A}$, respectively. The superscript $H$ and $T$ represent the
%conjugate transpose and transpose operation, respectively.

==> v 2.7_single_black/2_Systemmodel.tex <==
\section{Preliminaries}
\label{sec:Preliminaries}

\subsection{System Model}
\label{sec:System_Model}
% Structure:
% General overview; scenario, time, bandwidth, power etc.
% Arrival process at the transmitter, queue, QoS requirements, notation
% Operation of the transmitter and relays:
% Links of the broadcast and the relaying link, path loss, shadowing, {\rm{Pr}}^{{\rm{e}}} _j, SNR
% Packetization, error process, ARQ behavior (timing?), service process notation


We consider a simple relaying scenario with a source, a destination and a decode-and-forward (DF) relay as schematically
shown in Figure~\ref{system-instr}. 
\begin{figure}[!h]
\begin{center}
\includegraphics[width=0.55\linewidth, trim=10 20 10 20]{AWGN_relay.pdf}
%\includegraphics[width=0.9\linewidth, trim=0 650 90 0]{effectivecapacitymultirelay.eps}
\end{center}
\caption{Example of the considered single relay system scenario.}
\label{system-instr}
\end{figure}
The links between the above transceivers are referred to as the direct link  (from the
source to the destination), the backhaul link  (from the source to the relay) and the relaying link  (from
the relay to the destination). In general, we assume the direct link to be much weaker than the backhaul
link as well as the relaying link. 
The entire system operates in a slotted fashion  where time is divided into transmission periods of length $2m$ (symbols). Each transmission period contains two frames (each frame with length $m$),  which corresponds to the two hops of relaying.  The blocklength of the coding over the channel in each frame is as long as the frame length $m$. 

During a transmission period $i$, first a broadcasting frame is employed, followed by a relaying frame. In the broadcasting frame, the source transmits data to the relay and the destination. 
The received signals at the destination and the relay  in the broadcasting frame of transmission period $i$ are given by:
\begin{equation}
{\bf{y}}_{1,i}  = p_{\rm{tx}} {{{h}}_{1,i} } {\bf{x}}_i +{\bf{n}}_{1,i},
\end{equation}
\begin{equation}
{\bf{y}}_{2,i} =  p_{\rm{tx}} {h_{2,i} }  {\bf{x}}_i + {\bf{n}}_{2,i}.
\end{equation}
Next, if the data is decoded correctly and forwarded by the relay, the received signal at the destination  in the relaying frame  of transmission period $i$ is given by:
\begin{equation}
 {\bf{y}}_{3,i}  =   p_{\rm{tx}} {{h}}_{3,i}   {\bf{x}}_i  + {\bf{n}}_{3,i}.
\end{equation} 
The transmitted signal $\bf{x}$ and received signals ${\bf{y}}_{1,i}$, ${\bf{y}}_{2,i}$ and~${\bf{y}}_{3,i}$ are complex $m$-dimensional vectors.   Besides, the transmit power at either the relay or the source is denoted by $p_{\rm{tx}}$.   In addition, the noise vectors of these links in transmission period $i$ are denoted by ${\bf{n}}_{1,i}$, ${\bf{n}}_{2,i}$ and~${\bf{n}}_{3,i}$,  which are independent and identically distributed (i.i.d.) complex Gaussian vectors:   ${\bf{n}}$ $\! \sim \! {\mathcal{{N} }}\left( {0,{\sigma ^2}{{\bf{I}}_m}} \right)$,  $ {\bf{n}} \in \{{\bf{n}}_{1,i}, {\bf{n}}_{2,i}, {\bf{n}}_{3,i}\}$, where ${\bf{I}}_m$ denotes an $m \times m$ identity matrix.    
Moreover, ${{h}}_{1,i} $, $h_{2,i}$ and ${{h}}_{3,i}$ are the channels (scalars) of the direct link, backhaul link and relaying link during transmission period $i$, respectively. 
In this work, we consider quasi-static Rayleigh fading channels  where the channels remain constant within each transmission period (includes two hops/frames) and vary independently from one period to the next. 
{{{Hence, the instantaneous channel gain of each link  has two components, i.e., the average channel gain and the random fading. }}} 
On the one hand, {{{we denote  average channel gains (e.g., due to the path loss)  of these three links over the transmission periods by  $|{{\bar h}}_{2}|^2$, $|{{\bar h}}_{2}|^2$ and $|{{\bar h}}_{3}|^2$.}}}
On the other hand, we assume these channels to experience Rayleigh fading where the envelope $\sqrt z $ of the channel fading (response) is Rayleigh distributed with the probability density function (PDF) ${f}\left( {\sqrt z } \right) = 2 \frac{{\sqrt z }}{{{\sigma ^2}}}{e^{ - z/{\sigma ^2}}}$.
%In this work, we consider a Rayleigh quasi-static channel fading
%Hence, the envelope $\sqrt z $ of the channel fading (response) is Rayleigh distributed with the probability density function (PDF) ${f}\left( {\sqrt z } \right) = 2 \frac{{\sqrt z }}{{{\sigma ^2}}}{e^{ - z/{\sigma ^2}}}$. 
Typically, the channel fading is modeled as having unit power gain. This requires that $\sigma ^2 = 1$. Hence, 
the  PDF of  $z$, the gain due to Rayleigh fading, is given by the exponential distribution: $f( z ) = e^{ - z}$. {{{We denote by $z_{j,i}$ ($j = 1,2,3$)  the gains due to Rayleigh fading}}} (during transmission period $i$) of the direct link, the backhaul link and the relaying link.  
{{{Hence, we have $|h_{j,i}|^2 = {z_{j,i}}|{{\bar h}}_{j}|^2, j = 1,2,3$.}  Moreover, these channel fading gains at different links during the same transmission period are assumed to be independent and identically distributed (i.i.d). 


Finally, the destination is assumed to apply maximal ratio combining (MRC) 
 %based on the CSI
 where the combined channel gain is given by  $|{{ h}}_{1,i}|^2  + |{{ h}}_{3,i}|^2$.
Thus, the received signal-to-noise ratio (SNR) at the relay and the received SNR at the destination in  transmission period $i$ under maximum ratio combining are given by ${\gamma_{2,i}} = \frac{{{|{{ h}}_{2,i}|^2}{p_{{\rm{tx}}}}}}{{{\sigma ^2}}}$ and ${\gamma_{{\rm{MRC}},i}} = \frac{{\left( {{|{{ h}}_{1,i}|^2} + {|{{ h}}_{3,i}|^2}} \right){p_{{\rm{tx}}}}}}{{{\sigma ^2}}}$.



\subsection{Blocklength-Limited Performance of Single-Hop Transmission Scenario with Perfect CSI {{{(at the source)}}}}
 For  the real additive white Gaussian noise (AWGN) channel,~[8, Theorem 54] derives an accurate approximation of the
coding rate of a single-hop transmission system. With blocklength $m$, block error probability $\varepsilon$ and SNR $\gamma$, the coding rate (in bits per channel use) is given by:
 $r \approx \frac{1}{2}{\log _2}\left( {1 + \gamma } \right) - \sqrt {\frac{V_{\text{real}}}{m}} {Q^{ - 1}}\left( \varepsilon  \right)$, where~$Q^{ - 1}(\cdot)$ is the inverse Q-function, and as usual, the Q-function is given by $Q\left( w \right) = {\rm{ }}\int_w^\infty  {\frac{1}{{\sqrt {2\pi } }}} e^{ - t^2 /2} dt$. In addition, $V_{\text{real}}$ is the  channel dispersion of a real Gaussian channel which is given by $V_{\text{real}} = \frac{\gamma }{2}\frac{{\gamma  + 2}}{{{{\left( {1 + \gamma } \right)}^2}}}{\left( {{{\log }_2}e} \right)^2}$.
%Since $\frac{{\rm{O}}\left( {{{\log }_2}m} \right)}{m} \approx 0$, 
%{{It was reported in~\cite{Verdu_2010}  that the above approximation of  coding rate is accurate for AWGN channels.}} %for blocklengths and error probabilities of practical interest.}} 

{{Under a quasi-static fading channel model, each channel state  is assumed to be static during a transmission period.  Therefore, in each transmission period  a quasi-static fading channel with fading coefficient $h$ can be viewed as an AWGN channel with channel gain $|h|^2$.}} 
Therefore, the above result with a real AWGN channel can be reasonably extended to a complex quasi-static fading channel model  in~\cite{Yang_2014,Gursoy_2013,Peng_2011,Makki_2014,Makki_2015}: with a  channel gain~$|h|^2$ the coding rate of a transmission period (in bits per channel use) is given by: 
\begin{equation}
\label{eq:single_link_data_rate}
r =  {\rm{R}}({|h|^2},\varepsilon ,m)  \approx {\rm{C}}({|h|^2}) - \sqrt {\frac{{{V_{{\rm{comp}}}}}}{m}} {Q^{ - 1}}\left( \varepsilon  \right)\mathrm{,}
\end{equation}
where ${\rm{C}}\left( |h|^2 \right)$ is the  Shannon capacity function of a complex channel with gain~$|h|^2$: $ {\rm{C}}({|h|^2}) \!=\! {\log _2}\left( {1 + \frac{{{|h|^2}{p_{{\rm{tx}}}}}}{{{\sigma ^2}}}} \right)$. % \!=\! {\log _2}\left( {1 + \frac{{z{|h|^2}{p_{{\rm{tx}}}}}}{{{\sigma ^2}}}} \right)$.  
{{In addition,  the  channel dispersion of a complex Gaussian channel is  twice the one of a real Gaussian channel: ${V_{{\rm{comp}}}} = 2{V_{{\rm{real}}}} = \gamma \frac{{\gamma  + 2}}{{{{\left( {1 + \gamma } \right)}^2}}}{\left( {{{\log }_2}e} \right)^2} = \left( {1 - \frac{1}{{{{\left( {1 + \gamma } \right)}^2}}}} \right){\left( {{{\log }_2}e} \right)^2} = \left( {1 - {{\rm{2}}^{{\rm{ - 2C}}({|h|^2})}}} \right){\left( {{{\log }_2}e} \right)^2}$.}}

Then,  for a single hop transmission of a transmission period of quasi-static fading channel,  
with blocklength $m$ and coding  rate $r$, %if the transmitter has  perfect CSI,
 the decoding (block) error probability at the receiver is given by:  
\begin{equation}
\label{eq:single_link_error_pro}
\varepsilon  = {\rm{P}}({|h|^2},r,m)  \approx Q\left( {\frac{{{\rm{C}}({|h|^2}) - r}}{{\sqrt {{V_{{\rm{comp}}}}{\rm{/}}m} }}} \right).% = Q\left( {\frac{{{\rm{C}}({|h|^2}) - r}}{{\sqrt {\frac{1}{m}\left( {1 - {2^{ - 2{\rm{C}}({|h|^2})}}} \right)} {{\log }_2}e}}} \right).
\end{equation}

{{Considering the channel fading, the expected/average error probability over channel fading is given by~\cite{Yang_2014}:
\begin{equation}
\label{eq:expectedsingle_link_error}
\mathop {\mathop{\rm E}\nolimits} \limits_z \left[ \varepsilon  \right] = \mathop {\mathop{\rm E}\nolimits} \limits_z \left[ {{\rm{P}}(|h{|^2},r,m)} \right]  \approx \mathop {\mathop{\rm E}\nolimits} \limits_z \left[ {Q\left( {\frac{{{\rm{C}}(|h{|^2}) - r}}{{\sqrt {{V_{{\rm{comp}}}}{\rm{/}}m} }}} \right)} \right],
\end{equation}
where $\mathop {\mathop{\rm E}\nolimits} \limits_z \left[ *  \right]$ is the expectation over the distribution of channel fading gain $z$.}}

%As the Q-function is a strictly decreasing function, obviously ${\mathop{\rm P}}$  is strictly increasing in $r$ and  strictly decreasing in either $m$ or $|h|^2$. 


In the remainder of the paper,  {{{we investigate the blocklength-limited performance of relaying under quasi-static fading channels by  applying the above approximations.}}} As these approximations have been shown to be very tight for sufficiently large value of $m$~\cite{Verdu_2010,Polyanskiy_2011,Yang_2014}, for simplicity we will assume them to be equal in our analysis and numerical evaluation where we consider sufficiently large value of $m$ at each hop of relaying.



%{{In the remainder of the paper, we investigate the blocklength-limited performance of relaying under quasi-static fading channels by  applying approximation~\eqref{eq:single_link_data_rate} at the source (to determine the coding rate based on the average CSI) and applying approximation~\eqref{eq:expectedsingle_link_error} at each hop of relaying to address the average/expected error probability. As these approximations have been shown to
%be very tight for sufficiently large value of $m$~\cite{Verdu_2010,Polyanskiy_2011,Yang_2014}, for simplicity we will assume them to be equal in our analysis and numerical evaluation where we consider sufficiently large value of $m$ at each hop of relaying. }}




\section{Physical-layer Performance of Relaying with Average CSI}
\label{sec:Physical_layer_P}
With only average CSI, if the source determines the coding rate directly based on it, this  likely results in that $|{{ h}}_{j,i}|^2$, the instantaneous channel gain at transmission period $i$, is lower than  the average which is $|{{\bar h}}_{j}|^2$. And this leads to 
a  significant  error probability.
Therefore, % in order to avoid the high error probability, 
we propose the source to choose a relatively lower coding rate which is obtained by  the weighted  average channel gains $\eta |{{\bar h}}_{j}|^2$ ($j=1,2,3$), where  $\eta$  is a weight factor. In addition,  we assume that
%
 $0 < \eta  \le \hat z$, where $\hat z $ is the median of $z$.
{{ For link $j$, with probability  0.5 value $\eta$ is lower than the channel fading gain $z_j$,  i.e., ${\Pr} \{\eta < z_j\}  \le  0.5$.
Hence,  although the instantaneous channel gain $z_j |{{\bar h}}_{j}|^2$ is still possible  to be lower than the weighted one $\eta |{{\bar h}}_{j}|^2$, the probability of this becomes much lower when  $\eta< \hat z$ and is bounded by  0.5, i.e., ${\Pr} \{z_j |{{\bar h}}_{j}|^2 < \eta |{{\bar h}}_{j}|^2\} = {\Pr} \{\eta < z_j\}  \le   0.5$}}\footnote{The setup (letting $ {\hat z} $  be the upper limit of $\eta$) facilitates the proof of Theorem  1  and Theorem  2.  In addition, in practice it is unreasonable to choose a coding rate which  likely exceeds the Shannon limit with a probability higher than 0.5. Our setup just reduces this probability and bounds it by  0.5.    Hence, this setup is reasonable.
Moreover, we will also show in the simulation that this setup is not impacting the system operation/optimization as the optimal value of  $\eta$ is about 0.2 which is much lower than $\hat z \approx  0.7$ (Rayleigh channels).}.

Recall that we assume MRC to be applied at the destination. Hence, the coding rates at different hops of relaying are required to be the same.
{{This coding rate $r$ is  determined by the source based on the weighted average CSI according to~\eqref{eq:single_link_data_rate}.
 As the overall performance of the considered two-hop relaying system is actually mainly subject to the bottleneck link which is either the backhaul link or the combined link,  the coding rate is  determined by
$r = {\rm{R}}({\eta  \cdot \min \left\{{|{{\bar h}_2}{|^2},|{{\bar h}_{\rm{1}}}{|^2} + |{{\bar h}_{\rm{3}}}{|^2}} \right\}},\varepsilon^\circ,m)$, where $\varepsilon^\circ$ is a constant error probability and has a value of practical interest.}}
 According to~\eqref{eq:single_link_data_rate},  $r$ is strictly increasing in the weight factor~$\eta$. In other words, a big $\eta$ means a high expectation on the channel quality and results in a high coding rate. % In other words, $r$ is strictly increasing in $\eta$.  


Once the coding rate $r$ is determined, it will not be changed during transmission periods. In other words, from one transmission period to the next the coding rate is fixed  and therefore  error probabilities of different links  of relaying vary along with the channel fading.    
{{Regarding the overall error of relaying, in this work we treat the decoding error  at the destination based on the combined channel gain as the overall error. Although it is theoretically possible that an error occurs in the two-hop  relaying though  the direct transmission (in the broadcasting phase) is correct,  the probability of this is negligible as on the one hand we mainly consider  error probabilities of practical interest (which means  that the overall error probability of relaying is not significant) and on the other hand we assume the direct link to be much weaker than the backhaul
link as well as the relaying link.} 
Therefore, the overall error probability of relaying during transmission period~$i$ is given by:
%
\begin{equation}
\label{eq:Overall_error_pro}
{\varepsilon _{{\rm{R}},i}} = \varepsilon _{2,i} + \left( {1 - \varepsilon _{2,i}} \right) \cdot \varepsilon _{{\rm{MRC}},i} \mathrm{,}
\end{equation}
where $ \varepsilon _{{\rm{MRC}},i}= {\mathop{\rm P}} (|{{ h}}_{1,i}|^2 + |{{ h}}_{3,i}|^2,r,m)$ and $ \varepsilon _{2,i} =  {\mathop{\rm P}} (|{{ h}}_{2,i}|^2,r,m)$. 


Under the studied two-hop relaying scenario where the coding rate at each hop is $r$, the (source-to-destination) equivalent coding rate is actually $r/2$. Therefore, the expected BL-throughput of relaying during transmission period $i$ (the number of correctly received bits at the destination per channel use) is given by:
\begin{equation}
\label{eq:Overall_error_pro}
C_{{\rm{BL}},i}= r{(1-\varepsilon _{{\rm{R}},i})} /2  \mathrm{.}
\end{equation}
 
Then, we have the (average) BL-throughput of relaying over time, which is actually the expectation value of $C_{{\rm{BL}},i}$ over the transmission periods: 
\begin{equation}
\label{eq: BL-throughput_over_fading}
{C_{{\rm{BL}}}} = \mathop {\rm{E}}\limits_i \left[ {{C_{{\rm{BL}},i}}} \right] = r(1 - \mathop {\rm{E}}\limits_i \left[ {{\varepsilon _{{\rm{R}},i}}} \right])/2  \mathrm{.}
\end{equation}
 %As the BL-throughput$C_{{\rm{BL}}}$ is the average effectively transmitted information (per channel use) which is a very important performance metric. 
%Letting this BL-throughput of relaying as objective, we formulate the problem of this work as:
%\begin{equation}
%\begin{split}
%\mathop {\max }\limits_\eta \quad  &{C_{{\rm{BL}}}}\left( \eta  \right)\\
%s.t.: \quad & 0 < \eta  \le \hat z
%\end{split}
%\end{equation}

Hence, the major challenge for determining ${C_{{\rm{BL}}}}$ is to obtain  the expectation of  the overall error probability over the transmission periods, which is actually equal to the expectation over channel fading. 
Recall that all the channels are independent from each other, hence the expected value of the overall error probability of relaying is further given by: %can be obtained based on the expected value of error probability of each link:
\begin{equation}
\label{eq:mean_error_transfer}
\mathop {\rm{E}}\limits_i \left[ {{\varepsilon _{{\rm{R}},i}}} \right]  \!=  \!\! \! \! \mathop {\rm{E}}\limits_{{z_1},{z_2},{z_3}} \!\!\left[ {{\varepsilon _{\rm{R}}}} \right]  \!= \! \mathop {\rm{E}}\limits_{{z_2}}  \!\left[ {{\varepsilon _2}} \right]  + \! ( {1 - \mathop {\rm{E}}\limits_{{z_2}} \left[ {{\varepsilon _2}} \right]}   ) \!\mathop {\rm{E}}\limits_{{z_1},{z_3}} \left[ {{\varepsilon _{{\rm{MRC}}}}} \right] \mathrm{,}
\end{equation}
where $\mathop {\rm{E}}\limits_{{z_2}} \left[ {{\varepsilon _2}} \right]$ and $\mathop {\rm{E}}\limits_{{z_1},{z_3}} \left[ {{\varepsilon _{{\rm{MRC}}}}} \right]$ are the expectation values (over fading) of error probabilities of the backhaul link and the combined link.  {{Based on~\eqref{eq:expectedsingle_link_error}, they are given by:}}
\begin{equation}
\begin{split}
\mathop {\rm{E}}\limits_{{z_2}} \left[ {{\varepsilon _2}} \right] & = \int_0^\infty  {{e^{ - {z_2}}}} {\varepsilon _2}d{z_2}\\
& = {\int_0^\infty  {{\rm{P}}({z_2}|\bar h_2|^2,r,m){e^{ - {z_2}}}dz} _2}\\
& = \frac{1}{{\sqrt {2\pi } }}\int_0^\infty  {\int_{\sqrt m {{w}}({z_2})}^\infty  {{e^{ - \frac{{{t^2} + 2{z_2}}}{2}}}} } dtd{z_2}\mathrm{,}
\end{split}
\label{eq:expected_error_single_2}
\end{equation}
\begin{equation}
\begin{split}
\!\!\mathop {\rm{E}}\limits_{{z_1},\!{z_3}} \! \!\!\left[ {{\varepsilon _{{\rm{MRC}}}}} \right]\! &=\! \int_0^\infty   \! \!\! \!  \int_0^\infty \!   \!\! \! {\varepsilon _{{\rm{MRC}}}} {e^{ - {z_1} \!- {z_3}}}d{z_1}d{z_3}\\
 &=\!  \frac{1}{{\sqrt {2\pi } }}\! \! \int_0^\infty   \! \!\!\!  \int_0^\infty   \! \!\!\!  {\rm{P}}({z_1}|\bar h_1|^2 \!\! +\! {z_3}|\bar h_3|^2\! ,r\! ,m){e^{ \! - {z_1} \! - {z_3}}}d{z_1}d{z_3}\\
& =\!  \frac{1}{{\sqrt {2\pi } }}\! \! \! \int_0^\infty  \! \! \!\!  \int_0^\infty \!  \! \! \! \int_{\sqrt m {{w}}\left( {{z_1},{z_3}} \right)}^\infty \!\!\!\!  {e^{ - \frac{{{t^2} + 2{z_1} + 2{z_3}}}{2}}}dtd{z_1}d{z_3} \mathrm{,}
\end{split} 
\label{eq:expected_error_combine_link}
\end{equation}
where  $w\left( {{z_2}} \right) = \frac{{{\rm{C}}({z_2}|\bar h_2|^2) - r}}{{\sqrt {\frac{1}{m}\left( {1 - {2^{ - 2{\rm{C}}({z_2}|\bar h_2|^2)}}} \right)} {{\log }_2}e}}$ and ${{w}}({z_1},{z_3}) = \frac{{{\rm{C}}({z_1}|\bar h_1|^2 + {z_3}|\bar h_3|^2) - r}}{{\sqrt {\frac{1}{m}\left( {1 - {2^{ - 2 {\rm{C}}({z_1}|\bar h_1|^2 + {z_3}|\bar h_3|^2)}}} \right)} {{\log }_2}e}}$.

So far, we derived the  BL-throughput of relaying under the studied system. We then have the following theorem  regarding the BL-throughput.

\noindent
\textbf {Theorem  1 } \emph {Under a relaying scenario with quasi-static Rayleigh channels where only the average CSI is available at the source, % {{for  blocklengths of practical interest, i.e., $m \gg 1$,}} 
the  BL-throughput  is  concave in the coding rate.}

\begin{proof} {See Appendix A.}
\end{proof}
%

Recall that %the higher the weight factor $\eta$ is the higher the  coding rate the source chooses. In other words,
 the coding rate chosen by the source is strictly increasing in the weight factor $\eta$. Combined with   {Theorem~1}, we have an important corollary of Theorem  1:


\noindent
\textbf {Corollary 1} \emph {Consider a relaying scenario %{{with blocklengths of practical interest, i.e., $m \gg 1$,}} and 
with quasi-static Rayleigh channels while only the average CSI is available at the source.  If the source determines the coding rate according to the weighted average CSI,  the BL-throughput  is quasi-concave in the weight factor $\eta$.}

\begin{proof} {See Appendix B.}
\end{proof}

Therefore,  only with the average CSI there is a unique optimal value of $\eta$, which maximizes the  BL-throughput of relaying  {in}  the finite blocklength regime. 


%On the other hand, based on~\eqref{eq:single_link_error_pro} and~\eqref{eq:single_link_data_rate} both error probability and coding rate are influenced by the blocklength $m$. In particular, with a fixed coding rate at each link a long blocklength leads to a low error probability of each link. Obviously, this results in a low overall error probability of relaying. Based on the definition of BL-throughput, we immediately have the following theorem:

%\noindent
%\textbf {Theorem  2} \emph {Under a relaying scenario with quasi-static Rayleigh channels where only the average CSI is available at the source,  the  BL-throughput  is increasing  in the blocklength.}

\

\section{Link-Layer Performance of Relaying with Average CSI}
\label{sec:Higher_layer_P}
In this section, we study the Link-layer performance of relaying based on the \textit{effective capacity}, which is a well-known performance model that accounts for transmission and queuing effects in (wireless) networks~\cite{Dapeng_2003}.  We first briefly review the effective capacity model and extend the  expression of the maximum sustainable data rate into a  blocklength-limited relaying scenario. Subsequently, we derive the MSDR of the studied relaying system  {in}  the finite blocklength regime based on the model.

\subsection{Maximum Sustainable Data Rate}
\label{sec:ER_MSDR}

The effective capacity characterizes the (maximum) arrival rate of a flow to a queuing system and relates the stochastic characterization of the service of the queuing system to the queue-length or delay constraints of the flow. 
{{In}} the finite blocklength regime, decoding errors may occur. If a decoding error occurs in transmission period~$i$, the service process increment (effectively transmitted information)~$s_i$   of the two-frame relaying equals zero. 
On the contrary, if no error occurs at frame $i$, the service process increment equals $s_i = m   \cdot r$, where~$r$ is the coding rate (in bits per channel use) employed over a block of~$m$ symbols in each hop/frame of relaying.  
At period~$i$, the cumulative service process is $S_i = \sum_{n = 0}^{i} s_n$. Assume that the queue is stable as the average service rate is larger than the average arrival rate. Hence, the random queue length $Q_i$ at period $i$ converges to the steady-state random queue length $Q$. To characterize the long-term  statistics~$\mathrm{Pr}\left\{Q\right\}$ of the queue length, the framework of the effective capacity gives us the following upper bound:
\begin{equation}
\mathrm{Pr}\left\{Q > x\right\} \leq K \cdot e^{- \theta \cdot x }  \mathrm{,}
\label{eq:prob_bound}
\end{equation}
where $K$ is the probability that the queue is non-empty and $ \theta$ is the so called QoS exponent.
  Based on~\cite{kumar2004communication}, for a constant rate source with~$r$ bits per two-hop transmission period, the exponent $ \theta$ has to fulfill the following constraint:
\begin{equation}
r < - {{\Lambda \left( { - { \theta}} \right)} \mathord{\left/
 {\vphantom {{\Lambda \left( { - { \theta}} \right)} {{ \theta}}}} \right.
 \kern-\nulldelimiterspace} {{ \theta}}}  \mathrm{.}
\label{eq:qos_requirement}
\end{equation}
$\Lambda\left(\theta\right)$ is the log-moment generating
function of the cumulative service process~$S_i$
defined as:% (assuming the increments to be stationary as well):
\begin{equation}
\Lambda\left(\theta\right) = \lim_{i \to \infty} \frac{1}{i} \log \mathrm{E}\left[ e^{\theta \cdot \left(S_i - S_{0}\right)}\right] \! \mathrm{.}
\label{eqn:log_generating_function}
\end{equation}
The ratio $-\Lambda\left(-\theta\right) / \theta$ is called
the effective capacity.
%
% as the exponential decay of the distribution in Equation~\eqref{eq:prob_bound} is only witnessed if the ratio $\Lambda\left(-\theta\right) / \theta$ is bigger than the constant arrival rate $r$ of the source for some $ \theta$.
%
%So far we have only considered the random queue length. 
Denote by $D_i$ the random queuing delay of the head-of-line bit during period $i$. If the  constant arrival rate at the source  is  $r$, with a queue length of $Q = q$, a current delay of the head-of-line bit is given by $D = q/r$. This yields the following approximation for the steady-state delay distribution which is based on Equation~\eqref{eq:prob_bound}:
%
\begin{equation}
\mathrm{Pr}\left\{D > d\right\} \leq K \cdot e^{- \theta \cdot r \cdot d }  \mathrm{.}
\label{eq:prob_bound_specific}
\end{equation}
%
%A considerable challenge in determining the effective capacity is the characterization of  the log-moment generating function. 
If the service process $s_i$ can be assumed to be independent and identically distributed (i.i.d.),
a convenient simplification is to obtain the log-moment generating function via the {{{central limit theorem.}}}  %, {{i.e., as $i \to \infty$,  $S_i - S_{0}=\sum_0^i{s_i}$ becomes Gaussian-distributed.  In particular,  $\theta \sum\nolimits_0^i {{s_i}}  \sim {\mathscr N}\left( {i\theta {\mathop{\rm E}\nolimits} \left[ {{s_i}} \right],i{\theta ^2}{\rm    Var}\left[ {{s_i}} \right]} \right)$.
 Then, the effective capacity can be obtained by~\cite{Soret_2009}\footnote{{{{It should be mentioned that~\eqref{eq:single_channel_effective_capacity_central}  holds for i.i.d. $s_i$ but is just an approximation for general (non-i.i.d.) $s_i$}}}}:
\begin{equation}
-\frac{{\Lambda \left( { - \theta } \right)}}{\theta } \!=\!-\! \mathop {\lim }\limits_{i \to \infty } \frac{1}{{i\cdot\theta }}\log {\rm{E}}\left[ {{e^{ - \theta \cdot \sum\nolimits_1^i  {s_i}}}} \right] \!=\! \mathop {\rm{E}}\limits_i \left[ {{s_i}} \right] - \frac{\theta }{2}\mathop {{\rm{Var}}}\limits_i \left[ {{s_i}} \right].
\label{eq:single_channel_effective_capacity_central}
\end{equation}
Therefore, the queuing performance of the system is determined by the mean and the variance
of the random increment of the service process $s_i$. Combining~\eqref{eq:qos_requirement} and~\eqref{eq:prob_bound_specific}, the maximum arrival rate at the source $R_{\rm MS}$ in (bits per transmission period) that can be supported by the random service process  is obtained,  which has been first proposed by~\cite{Soret_2010}:
$ \frac{{\mathop {\rm{E}}\limits_i \left[ {{s_i}} \right]}}{2} + \frac{1}{2}\sqrt {{{( {\mathop {\rm{E}}\limits_i \left[ {{s_i}} \right]} )}^2} + \frac{{2\ln \left( {{P_{\rm{d}}  }} \right)}}{d}\cdot\mathop {{\rm{Var}}}\limits_i \left[ {{s_i}} \right]}$. In the formula, ${\left\{{d,P_{\rm{d}} } \right\}}$ is  QoS requirement pair of the service, where in~\cite{Soret_2010} $d$  is the delay constraint with transmission period as unit and $P_{\rm{d}}$ is the constraint of delay violation probability.
%Hence, the maximum arrival rate at the source $R_{\rm MS}$ in (bits per transmission period) that can be supported by the random service process  is obtained  by combining~\eqref{eq:qos_requirement} and~\eqref{eq:prob_bound_specific}, which has been first proposed by~\cite{Soret_2010}: $ \frac{{\mathop {\rm{E}}\limits_i \left[ {{s_i}} \right]}}{2} + \frac{1}{2}\sqrt {{{\left( {\mathop {\rm{E}}\limits_i \left[ {{s_i}} \right]} \right)}^2} + \frac{{2\ln \left( {{P_{\rm{d}}  }} \right)}}{d}\cdot\mathop {{\rm{Var}}}\limits_i \left[ {{s_i}} \right]}$.

The above maximum source rate  is the so-called maximum sustainable data rate (MSDR) and in this work we refer to MSDR as the metric of link-layer performance. 
Now, we extend the above MSDR into the studied relaying system  {in}  the finite blocklength regime. First, we redefine the unit of the delay constraint $d$ and let $d$ be in symbols.
Recall that in the studied system the length of each (two-hop relaying) transmission period is~$2m$. Therefore,  the delay constraint is $d/2m$  times of a transmission period. Then, the MSDR (bits per channel use)  of the studied two-hop relaying system is given by:
 %The number of transmission frames (including retransmissions for decoding errors) of a data packet should be lower than $d/m$. 
\begin{equation}
 {R_{\rm MS} } \! \approx \! \frac{{\mathop {\rm{E}}\limits_i \left[ {{s_i}} \right]}}{4m} \!+ \! \frac{1}{4m}\sqrt {{{\left( {\mathop {\rm{E}}\limits_i \left[ {{s_i}} \right]} \right)}^2} \!+\! \frac{{4m\ln \left( {{P_{\rm{d}}  }} \right)}}{d}\!\cdot\!\mathop {{\rm{Var}}}\limits_i \left[ {{s_i}} \right]}  \mathrm{.}
\label{eq:rate_function_general}
\end{equation}
Based on~\eqref{eq:rate_function_general}, the major challenge for determining the MSDR ${R_{\rm MS}}$ is to obtain the mean and variance of the service process  increment of the studied relaying system.


\subsection{Mean and Variance of the Service Process Increment}

Recall that the service process increment of a transmission period  is either zero or $rm$. In other words, it is  Bernoulli-distributed. Moreover, the probability of the error event of this Bernoulli distribution is actually the expected overall error probability of relaying which was given in the previous section by~\eqref{eq:mean_error_transfer}.
Based on the characteristic of the Bernoulli distribution, we immediately have the mean and variance of  service process increments:
\begin{equation}
\label{eq:mean_final}
\mathop {\rm{E}}\limits_i \left[ {{s_i}} \right]= rm \cdot (1 - \mathop {\rm{E}}\limits_{{z_1},{z_2},{z_3}} \left[ {{\varepsilon _{\rm{R}}}} \right])  \mathrm{,}
\end{equation}
%
\begin{equation}
\label{eq:var_final}
\mathop {{\rm{Var}}}\limits_i \left[ {{s_i}} \right] = {r^2}{m^2}\mathop {\rm{E}}\limits_{{z_1},{z_2},{z_3}} \left[ {{\varepsilon _{\rm{R}}}} \right] \cdot (1 -\mathop {\rm{E}}\limits_{{z_1},{z_2},{z_3}} \left[ {{\varepsilon _{\rm{R}}}} \right]) .
\end{equation}
%where the overall error probability (of relaying over channel fading) $\mathop {\rm{E}}\limits_{{z_1},{z_2},{z_3}} \left[ {{\varepsilon _{\rm{R}}}} \right]$ was given in the previous section by~\eqref{eq:mean_error_transfer}.

Substituting~\eqref{eq:mean_final} and~\eqref{eq:var_final} into~\eqref{eq:rate_function_general}, we have
\begin{equation}
\label{eq:MSDR_final}
{R_{{\rm{MS}}}} = \frac{{r(1 - \mathop {\rm{E}}\limits_{{z_1}\!,{z_2}\!,{z_3}\!} \left[ {{\varepsilon _{\rm{R}}}} \right])}}{4}  + \frac{r}{4}\sqrt {{{( {1 \!-\!\! \mathop {\rm{E}}\limits_{{z_1}\!,{z_2}\!,{z_3}\!} \left[ {{\varepsilon _{\rm{R}}}} \right]} )}^2} \!\!\!+\! \frac{{4m\ln \left( {{P_{\rm{d}}}} \right)}}{d} \!\!\!\!\mathop {\rm{E}}\limits_{{z_1}\!,{z_2}\!,{z_3}\!} \left[ {{\varepsilon _{\rm{R}}}} \right](1 \!-\!\!\! \mathop {\rm{E}}\limits_{{z_1}\!,{z_2}\!,{z_3}\!} \left[ {{\varepsilon _{\rm{R}}}} \right])} .
\end{equation}

Obviously, the performance of  MSDR $ {R_{\rm MS} }$ is subject to the coding rate $r$, as ${\mathop {\rm{E}}\limits_i \left[ {{\varepsilon _{{\rm{R}},i}}} \right]}$ is also a function of $r$. In fact, the following theorem  holds regarding the relationship between MSDR and the coding rate.

\noindent
\textbf {Theorem  2} \emph {Under a relaying scenario with quasi-static Rayleigh channels where only the average CSI is available at the source,  
%{{for blocklengths of practical interest, i.e., $m \gg 1$,}}
 the  MSDR is concave in the coding rate $r$.}

\begin{proof} {See Appendix D.}
\end{proof}


Similar to Theorem  1, Theorem  2 has the following corollary:

\noindent
\textbf {Corollary 2 } \emph {Consider a relaying scenario   %{{with blocklengths of practical interest, i.e., $m \gg 1$,}} and 
with quasi-static Rayleigh channels while only the average CSI is available at the source.  If the source determines the coding rate according to the weighted average CSI, the MSDR  is quasi-concave in the weight factor $\eta$.}
\begin{proof} {The proof of Corollary 2 (based on  Theorem  2) is similar to the proof of  Corollary~1 (based on  Theorem~1).}
\end{proof}

Hence, the {{link}}-layer performance MSDR also can be optimized by choosing an appropriate~$\eta$. %This is an important guideline for the system design.


%\noindent
%\textbf {Theorem  5} \emph {Under a relaying scenario with quasi-static Rayleigh channels where only the average CSI is available at the source, the  MSDR  is quasi-concave in the blocklength $m$.}


==> v 2.7_single_black/3_Overall_rate.tex <==

In~\eqref{eq:Overall_error_pro}, the relationship between the overall error probability and the error probability of single links is presented. From~\eqref{eq:single_link_error_pro}, the  error probability of a single link is subject to the related  raw rate . Therefore, in the following we further investigate the overall error probability by determining the overall  raw rate . 
As the channel information of all the three links are available at the source, the source is able to choose the  raw rate  which fulfills the channel conditions. 
As the  raw rate  of the two phases are the same, the source determines the  raw rate  of each frame 
based on the bottleneck link which is either the backhaul link or the combined link.
In other words, the  raw rate  is subject to  $\min \{{\bf{h}}_2^2, {\bf{h}}_1^2  + {\bf{h}}_3^2 \}$. 
%%Obviously, the overall error probability is subject to the channel qualities: ${\bf{h}}_1^2 $, ${\bf{h}}_2^2 $ and ${\bf{h}}_3^2 $. Firstly, ${\bf{h}}_1^2  + {\bf{h}}_3^2 $ determine the received SNR at the destination, it directly affects the decoding error probability at destination. Secondly, the relay cannot forward the data packet if error decoding happens at it,  which rapidly reduce the received SNR at the destination. In other words, ${\bf{h}}_2^2 $ affects the overall performance indirectly. %  Note that the raw  rate of all the three links should be the same.  
%Therefore, either  ${\bf{h}}_1^2  + {\bf{h}}_3^2 $ (directly) or ${\bf{h}}_2^2 $ is able to restrict the system performance. 
%
%Regarding the relationship  between $ {\bf{h}}_2^2$ and ${\bf{h}}_1^2  + {\bf{h}}_3^2$, 
We therefore investigate the overall error probability based on the following two cases:
\begin{itemize}
\item  {\bf{Case 1}}: ${\bf{h}}_2^2   \ge {\bf{h}}_1^2   + {\bf{h}}_3^2  $, which means the relay backhaul (source-relay) link is stronger than the combined link to the destination. If the target error probability of the combined link is set as ${{{\Pr}}}^{{\rm{e}}}_{\rm{co}}$, % from~\eqref{eq:single_link_data_rate} the  raw  rate of each phase $r$ can be determined based on the combined channel gain ${\bf{h}}_1^2 + {\bf{h}}_3^2 $. Hence,
 the overall  raw  rate decided by the source can be expressed as $r_{\rm{RA}}  = {\frac{1}{2}} r({\bf{h}}_1^2   + {\bf{h}}_3^2 , {{{\Pr}}}^{{\rm{e}}}_{\rm{co}},2m )$. Hence, the relative overall error probability is a function of  ${\Pr} _{{\rm{co}}}^{\rm{e}}$ and is obtained by:
\begin{equation}
\label{eq:error_pro1}
{\Pr} _{{\rm{RA}}}^{\rm{e}}({\Pr} _{{\rm{co}}}^{\rm{e}}) = {{\Pr} ^{\rm{e}}}\left( {{\bf{h}}_2^2,2{r_{{\rm{RA}}}},2m} \right) + \left( {1 - {{{\Pr} }^{\rm{e}}}\left( {{\bf{h}}_2^2,2{r_{{\rm{RA}}}},2m} \right)} \right) \cdot {\Pr} _{{\rm{co}}}^{\rm{e}} \mathrm{.}
 \end{equation}
Then ${{{\Pr}}}^{{\rm{e}}} [{\bf{h}}_2^2  ,r({\bf{h}}_1^2   + {\bf{h}}_3^2  , {{{\Pr}}}^{{\rm{e}}}_{\rm{co}} )] \le  {{{\Pr}}}^{{\rm{e}}}_{\rm{co}}$, hence we have:
\begin{equation}
\label{eq:upperboundOverall_error_pro1}
%{{{\Pr}}}_{\rm{co}}^{{\rm{e}}}\le 
{{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}  ( {{{\Pr}}}^{{\rm{e}}}_{\rm{co}} ) \le 
2{{{\Pr}}}_{{\rm{co}}}^{\rm{e}}  - \left( {{{{\Pr}}}_{{\rm{co}}}^{\rm{e}} } \right)^2 \mathrm{.}
\end{equation}
Especially, ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}} \! ( {{{\Pr}}}^{{\rm{e}}}_{\rm{co}} )\! \approx \!  {{{\Pr}}}^{{\rm{e}}}_{\rm{co}} $ when ${\bf{h}}_2^2   \gg   {\bf{h}}_1^2   + {\bf{h}}_3^2 $.
\item {\bf{Case 2}}:  ${\bf{h}}_2^2   < {\bf{h}}_1^2   + {\bf{h}}_3^2  $, the bottleneck link is the backhaul link. % Hence, the overall  raw  rate can be determined based on the backhaul channel gain ${\bf{h}}_2^2 $ and the related target error probability ${{{\Pr}}}_2^{{\rm{e}}}$.
 In this case, $r_{\rm{RA}}  = {\frac{1}{2}} r({\bf{h}}_2^2  ,{{{\Pr}}}_2^{{\rm{e}}},2m )$ while the overall error probability is the function of ${{{\Pr}}}_2^{{\rm{e}}}$:
\begin{equation}
\label{eq:error_pro2}
\!{{{\Pr}}}^{{\rm{e}}} _{\rm{RA}} ({{{\Pr}}}_2^{{\rm{e}}}) \! =\! {{{\Pr}}}_2^{{\rm{e}}} + 
 \left( {1 \! -\! {{{\Pr}}}_2^{{\rm{e}}} } \right)\cdot {{{\Pr}}}^{{\rm{e}}} \left( {{\bf{h}}_1^2  \!+\! {\bf{h}}_3^2  ,r_{\rm{RA}},2m} \right) \mathrm{.}
\end{equation}

Similarly, the upper bound of ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}$ can be given by:
\begin{equation}
\label{eq:upperboundOverall_error_pro2}
%{{{\Pr}}}_2^{{\rm{e}}}\le
{{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}  ({{{\Pr}}}_2^{{\rm{e}}} ) \le
2{{{\Pr}}}_2^{\rm{e}}  - \left( {{{{\Pr}}}_2^{\rm{e}} } \right)^2 \mathrm{.}
\end{equation}
Especially, ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}} ({{{\Pr}}}_2^{{\rm{e}}} ) \approx {{{\Pr}}}_2^{{\rm{e}}} $ when $  {\bf{h}}_1^2   + {\bf{h}}_3^2  \gg {\bf{h}}_2^2  $.
\end{itemize}

%Firstly, the overall probability is  strongly subject to the error probability target of the bottleneck  link.
Section~\ref{sec:The_Effective_Rate} will show that by choosing an appropriate error probability target for the bottleneck link, the BL-capacity of the system is able to be maximized. 



Firstly, combining~\eqref{eq:upperboundOverall_error_pro1} and~\eqref{eq:upperboundOverall_error_pro2} with~\eqref{eq:LowerboundOverall_error_pro}, the overall error probability of relaying can be bounded by:
\begin{equation}
\label{eq:final_bounds}
2{{\Pr}}_j^{\rm{e}}  - \left( {{{\Pr}}_j^{\rm{e}} } \right)^2  \ge {{\Pr}}_{{\rm{RA}}}^{\rm{e}}  \ge {{\Pr}}_j^{\rm{e}} \; \mathrm{,}
\end{equation}
where ${\Pr} _j^{\rm{e}}  = \max \{ {{\Pr}}_{{\rm{co}}}^{\rm{e}} ,{\Pr} _2^{\rm{e}} \} $ is the error probability of the bottleneck link:  ${{{\Pr}}}^{{\rm{e}}} _j= {{{\Pr}}}^{{\rm{e}}} _{\rm{co}}$ if $ {\bf{h}}_2^2   \ge {\bf{h}}_1^2   + {\bf{h}}_3^2 $ and  ${{{\Pr}}}^{{\rm{e}}} _j= {{{\Pr}}}^{{\rm{e}}} _{2}$ if $ {\bf{h}}_2^2   <{\bf{h}}_1^2   + {\bf{h}}_3^2 $.
%\begin{equation}
% {{{\Pr}}}^{{\rm{e}}} _j= \left\{ { \begin{array}{*{20}c}
 %  {{{\Pr}}}^{{\rm{e}}} _{\rm{co}} & {if \; {\bf{h}}_2^2   \ge {\bf{h}}_1^2   + {\bf{h}}_3^2  }  \\
  % {{{\Pr}}}^{{\rm{e}}} _2 & {if \; {\bf{h}}_2^2   < {\bf{h}}_1^2   + {\bf{h}}_3^2  }  \\
%\end{array}} \right. \; \mathrm{.}
%\end{equation}




Secondly, the overall  raw rate  can be given based on the function of~\eqref{eq:single_link_data_rate} by: 
\begin{equation}
\label{eq:overalldatarate}
% r_{\rm{RA}}= \left\{ { \begin{array}{*{20}c}
%   {\frac{1}{2}} r({\bf{h}}_1^2   + {\bf{h}}_3^2 , {{{\Pr}}}^{{\rm{e}}}_{\rm{co}} ) & {if \; {\bf{h}}_2^2   \ge {\bf{h}}_1^2   + {\bf{h}}_3^2  }  \\
%   {\frac{1}{2}} r({\bf{h}}_2^2  ,{{{\Pr}}}_2^{{\rm{e}}} ) & {if \; {\bf{h}}_2^2   < {\bf{h}}_1^2   + {\bf{h}}_3^2  }  \\
%\end{array}} \right.
r_{{\rm{RA}}}  = 0.5 r\left( {\min \left\{ {{\bf{h}}_2^2 ,{\bf{h}}_1^2  + {\bf{h}}_3^2 } \right\}, \max \left\{ {{\Pr} _2^{\rm{e}} ,{\Pr} _{{\rm{co}}}^{\rm{e}} } \right\}}, 2m \right)\mathrm{.}
\end{equation}

%Obviously, for fixed channel conditions, the overall  raw rate  is totally subject to the error probability of the bottleneck link.
Thirdly,~\eqref{eq:error_pro1} and~\eqref{eq:error_pro2} show that the overall error probability ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}$ is fully determined by the overall  raw rate  $r _{\rm{RA}}$. 
It is also shown in~\eqref{eq:overalldatarate} that for fixed channel conditions $r _{\rm{RA}}$ is further totally subject to the error probability of the bottleneck link ${{{\Pr}}}^{{\rm{e}}} _j$.
As a result, ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}$ is completely subject to ${{{\Pr}}}^{{\rm{e}}} _j$.
In other words, with non-fading channels the system is able to achieve the target overall error probability by choosing an appropriate  value of ${{{\Pr}}}^{{\rm{e}}} _j$.
In fact, ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}({{{\Pr}}}^{{\rm{e}}} _j)$ has the following characteristic:
%The relationship between them are presented in the Proposition 2.
%
%Then, for a target overall error probability $\hat{{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}$, the overall maximal achievable rate can be modeled as the follow problem: 
%\begin{equation}
%\begin{array}{l}
% \mathop {\max } \limits_{{{{\Pr}}}^{{\rm{e}}} _j } {r_{\rm{RA}} ({{{\Pr}}}^{{\rm{e}}} _j) } \\ 
% s.t.: \; {{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}  \left( {{{{\Pr}}}^{{\rm{e}}} _j } \right) \le \hat {{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}   \\ 
% \end{array} \; \mathrm{.}
%\end{equation}
%
%Obviously, $r_{\rm{RA}} $ is an increasing function in ${{{\Pr}}}^{{\rm{e}}} _j$, hence the solution to the above problem is equivalent to the solution to the follow problem: 
%\begin{equation}
%\begin{array}{l}
% \mathop {\max }{{{{\Pr}}}^{{\rm{e}}} _j }  \\ 
% s.t.: \; {{{\Pr}}}^{{\rm{e}}} _{\rm{RA}} \left( {{{{\Pr}}}^{{\rm{e}}}_j } \right) \le \hat{{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}  \\ 
% \end{array} \; \mathrm{.}
%\end{equation}
%\newtheorem{theorem2}{Proposition}
%\begin{theorem2}
%if the $ {\rm{ }}\frac{{xP_{{\rm{tx}}} }}{{\sigma ^2 }} > 0$~$dB$ $\forall$ $x={\bf{h}}_1^2 $, ${\bf{h}}_2^2 $ and ${\bf{h}}_3^2 $,   $\varepsilon _{\rm{O}} (\varepsilon _i )$ is increasing in $\varepsilon _i$.
%\label{th:monn-dec2}
%\end{theorem2}
\

\noindent
\textbf {Proposition 2 } \emph {The overall error probability ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}  ({{{\Pr}}}^{{\rm{e}}} _j )$ is strictly increasing in ${{{\Pr}}}^{{\rm{e}}} _j$. }


We provide here the proof under the assumption that ${\bf{h}}_2^2   \ge {\bf{h}}_1^2   + {\bf{h}}_3^2 $, the other situation can be proved similarly.
\begin{proof}
$\because$  ${\bf{h}}_2^2   \ge {\bf{h}}_1^2   + {\bf{h}}_3^2 $% , the overall probability is given by 

$\therefore$ ${{\Pr}}_{{\rm{RA}}}^{\rm{e}}({{{\Pr}}}_{{\rm{co}}}^{\rm{e}} )  = {{\Pr}}^{\rm{e}} [{\bf{h}}_2^2 ,r({\bf{h}}_1^2  + {\bf{h}}_3^2 ,{{\Pr}}_{{\rm{co}}}^{\rm{e}},2m )] + \left( {1 - {{\Pr}}^{\rm{e}} [{\bf{h}}_2^2 ,r({\bf{h}}_1^2  + {\bf{h}}_3^2 ,{{\Pr}}_{{\rm{co}}}^{\rm{e}},2m )]} \right)\cdot {{\Pr}}_{{\rm{co}}}^{\rm{e}} $.




$\therefore$ the derivative of ${{\Pr}}_{\rm{RA}}^{\rm{e}}$ with respect to ${{\Pr}}_{\rm{co}}^{\rm{e}}$ can be obtained by:
%
\begin{equation}
\label{eq:derivativesOverallPr_co}
  \frac{{\partial {{\Pr}}_{{\rm{RA}}}^{\rm{e}} ({{{\Pr}}}_{{\rm{co}}}^{\rm{e}} )}}{{\partial {{{\Pr}}}_{{\rm{co}}}^{\rm{e}} }}= \frac{{\partial {{{\Pr}}}_{{}}^{\rm{e}} ({{{\Pr}}}_{{\rm{co}}}^{\rm{e}} )}}{{\partial r}}\frac{{\partial r}}{{\partial {{{\Pr}}}_{{\rm{co}}}^{\rm{e}} }} 
=\left[ {\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{}} }}\left( {1 - {{\Pr}}_2^{\rm{e}} } \right) + \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{}} }}\left( {1 - {{\Pr}}_{{\rm{co}}}^{\rm{e}} } \right)} \right]\frac{{\partial r}}{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }} \; \mathrm{.}
\end{equation}


$\because$ $r({\bf{h}}_1^2   + {\bf{h}}_3^2  , {{{\Pr}}}^{{\rm{e}}}_{{\rm{co}}},2m )$ is the increasing in $ {{{\Pr}}}^{{\rm{e}}}_{{\rm{co}}}$ as well as ${{{\Pr}}}^{{\rm{e}}} (x, r, 2m)$ is increasing in $ r$,

$\therefore$ $\frac{{\partial {{{\Pr}}}_1^{\rm{e}} }}{{\partial r}} > 0$, $\frac{{\partial {{{\Pr}}}_2^{\rm{e}} }}{{\partial r}} > 0$ and $\frac{{\partial r}}{{\partial {{{\Pr}}}_{{\rm{co}}}^{\rm{e}} }}> 0$.

%$\because$ ${\bf{h}}_1^2   + {\bf{h}}_3^2 \ge {\bf{h}}_1^2$,

%$\therefore$ ${{\rm{Pr}}_1^{\rm{e}}  \ge {\rm{Pr}}_{{\rm{co}}}^{\rm{e}} }$.
 
$\because$ $0 \le {\rm{Pr}}_2^{\rm{e}}  \le 1$ and $0 \le {\rm{Pr}}_{\rm{co}}^{\rm{e}}  \le 1$

$\therefore$ based on~\eqref{eq:derivativesOverallPr_co}, ${{\partial \Pr _{{\rm{RA}}}^{\rm{e}} (\Pr _{{\rm{co}}}^{\rm{e}} )} \mathord{\left/
 {\vphantom {{\partial \Pr _{{\rm{RA}}}^{\rm{e}} (\Pr _{{\rm{co}}}^{\rm{e}} )} {\partial \Pr _{{\rm{co}}}^{\rm{e}} }}} \right.
 \kern-\nulldelimiterspace} {\partial \Pr _{{\rm{co}}}^{\rm{e}} }} > 0$.

$\therefore$ ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}  ({{{\Pr}}}^{{\rm{e}}} _{{\rm{co}}} )$ is strictly increasing in ${{{\Pr}}}^{{\rm{e}}} _{{\rm{co}}}$.
\end{proof}

So far, the overall  raw rate  and the overall error probability have been investigated for the relay system  with non-fading channels. Based on this, we  study the BL-capacity of the relay system under the finite blocklength regime.
%


\subsection{The BL-capacity}
\label{sec:The_Effective_Rate}

Based on~\eqref{eq:single_link_data_rate}, the raw rate of each phase $r$ is increasing in ${{{\Pr}}}^{{\rm{e}}} _j$. Therefore,  $r_{\rm{RA}}$ is also increasing in ${{{\Pr}}}^{{\rm{e}}} _j$ since $r_{\rm{RA}}=r/2$.
%Therefore, both the overall maximal rate $r_{\rm{RA}}$  and the overall error probability ${{{\Pr}}}^{{\rm{e}}}_{\rm{RA}}$ are increasing in ${{{\Pr}}}^{{\rm{e}}}_j$ the error probability of bottleneck link. 
Hence, the overall  raw rate  $r_{\rm{RA}}$  tends to infinity as long as ${{{\Pr}}}^{{\rm{e}}} _j$ goes to $1$. At the same time, the overall error probability also tends to 1. Note that the overall    raw rate  is not a successfully received/decoded data rate but a data rate based on the pure physical attempt to transmit bits from the source. So the destination decodes nothing correctly if the overall error probability is~1. Therefore, in order to investigate the effective performance of the relay system, it is more~meaningful to consider the correctly received data rate -- the BL-capacity. 
 % where the overall error probability is higher than 0.5. 

The service process $s_i$ of frame~$i$ (in bits per m channel use) is given based on the overall  raw rate :
\begin{equation}
s_i  = 2m \varphi r_{\rm{RA}}.
\end{equation}
where $\varphi$ is a binary random variable defined by  ${\Pr} \{ \varphi  = 1\}  = {1 - {{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}  }$ and ${\Pr} \{ \varphi  = 0\}  = { {{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}}$.
% 
Therefore, the BL-capacity, which is the expected value of the service process $s_i$,  is given by:
\begin{equation}
{\rm{E}}\left[ {s_i } \right] =  2\left( {1 -  {{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}  } \right)m \cdot  r_{\rm{RA}}\mathrm{.}
\label{eq:mean}
\end{equation}
We then have the following proposition on the BL-capacity:

%\

\noindent
\textbf {Proposition 3 } \emph {The BL-capacity ${\rm{E}}\left[ {s_i } \right]$ is a concave function in the overall  raw rate  $r_{\rm{RA}}$.}

Here we provide the proof under the situation that the bottleneck link is the backaul link, the other situation can be analyzed similarly. In addition, 
to simplify the proof of the proposition, we do not consider the extreme error situation.









%Therefore, the long expression of $\frac{{\partial {\rm{E}}\left[ {s_i } \right]}}{{\partial r_{{\rm{RA}}} }}$ can be divided into two parts:
%\begin{equation}
%\frac{{\partial {\rm{E}}\left[ {s_i } \right]}}{{\partial r_{{\rm{RA}}} }}={\mathop{\rm f}\nolimits} _{{\rm{In}}} \left( {r_{{\rm{RA}}} } \right) + {\mathop{\rm f}\nolimits} _{{\rm{De}}} \left( {r_{{\rm{RA}}} } \right)
%\end{equation}
%where ${\mathop{\rm f}\nolimits} _{{\rm{In}}} \left( {r_{{\rm{RA}}} } \right) $  and ${\mathop{\rm f}\nolimits} _{{\rm{De}}} \left( {r_{{\rm{RA}}} } \right)$ are the increasing part and decreasing part of the $\frac{{\partial {\rm{E}}\left[ {s_i } \right]}}{{\partial r_{{\rm{RA}}} }}$:
%\begin{equation}
%{\mathop{\rm f}\nolimits} _{{\rm{In}}} \left( {r_{{\rm{RA}}} } \right) = mr_{{\rm{RA}}} {{\Pr}}_{{\rm{co}}}^{\rm{e}} \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + mr_{{\rm{RA}}} \frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} {{\Pr}}_2^{\rm{e}} 
%\end{equation}
%\begin{equation}
%{\mathop{\rm f}\nolimits} _{{\rm{De}}} \left( {r_{{\rm{RA}}} } \right) = \left( {1 - {{\Pr}}_{{\rm{RA}}}^{\rm{e}} } \right)m - mr_{{\rm{RA}}} \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} - mr_{{\rm{RA}}} \frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}
%\end{equation}
%Then we get the relative derivatives of two parts with respective to $r_{\rm{RA}}$: 
%\begin{equation}
%\begin{array}{l}
% \frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{In}}} }}{{\partial r_{{\rm{RA}}} }} = m{\Pr} _{{\rm{co}}}^{\rm{e}} \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + m\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}{\Pr} _2^{\rm{e}}  \\ 
%  + mr_{{\rm{RA}}} \left( {2\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + {{\Pr}}_{{\rm{co}}}^{\rm{e}} \frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} + {{\Pr}}_2^{\rm{e}} \frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}} \right) \\ 
% \end{array}
%\end{equation}

%\begin{equation}
%\begin{array}{l}
% \frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{De}}} }}{{\partial r_{{\rm{RA}}} }} =  - 2m\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} - 2m\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + m{\Pr} _{{\rm{co}}}^{\rm{e}} \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + m{\Pr} _2^{\rm{e}} \frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} \\ 
 % - mr_{{\rm{RA}}} \left( {\frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} + \frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}} \right) \\ 
 %\end{array}
%\end{equation}

%Consider that 

%$\mathop {\lim }\limits_{r_{{\rm{RA}}}  \to 0} \frac{{\partial {\rm{E}}\left[ {s_i } \right]}}{{\partial r_{{\rm{RA}}} }} = m > 0$, therefore the following proposition holds if $\frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{In}}} }}{{\partial r_{{\rm{RA}}} }} < - {\frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{De}}} }}{{\partial r_{{\rm{RA}}} }}}$ where $r_{\rm{RA}}\in (0, \mathop {\min }\limits_{x_j  \in \left\{ {z_2 ,z_{co} } \right\}} \left\{ {\frac{1}{2}c\left( {x_j } \right)} \right\})$.

%\noindent
%\textbf {Proposition 3 } \emph {The mean of service rate ${\rm{E}}\left[ {s_i } \right]$ is a convex function of the overall  raw rate  $r_{\rm{RA}}$, $r_{\rm{RA}}\in (0, \mathop {\min }\limits_{x_j  \in \left\{ {z_2 ,z_{co} } \right\}} \left\{ {\frac{1}{2}c\left( {x_j } \right)} \right\})$.}




%\begin{proof}

%\noindent

%$\because$ ..XXXXXXXXXXXXXXXXXXXXXX


%$\therefore$  $-\frac{{\partial^2 {\mathop{\rm f}\nolimits} _{{\rm{De}}} }}{{\partial^2 r_{{\rm{RA}}} }} \ge  \frac{{\partial^2 {\mathop{\rm f}\nolimits} _{{\rm{In}}} }}{{\partial^2 r_{{\rm{RA}}} }}$

%$\because$ $\begin{array}{l}
%\mathop {\lim }\limits_{r_{{\rm{RA}}}  \to 0} \frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{In}}} }}{{\partial r_{{\rm{RA}}} }} = \mathop {\lim }\limits_{r_{{\rm{RA}}}  \to 0} - \frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{De}}} }}{{\partial r_{{\rm{RA}}} }} \\
%= m\left( {\mathop {\lim }\limits_{r_{{\rm{RA}}}  \to 0} \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + \mathop {\lim }\limits_{r_{{\rm{RA}}}  \to 0} \frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}} \right)\\
%\end{array}$

%$\therefore$  $\frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{In}}} }}{{\partial r_{{\rm{RA}}} }} < - {\frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{De}}} }}{{\partial r_{{\rm{RA}}} }}}$ when $r_{\rm{RA}}\in (0, \mathop {\min }\limits_{x_j  \in \left\{ {z_2 ,z_{co} } \right\}} \left\{ {\frac{1}{2}c\left( {x_j } \right)} \right\})$.  
%
%\end{proof}



%%%%%%%%%%%%%%%%%%%%%%proof%%%%%%%%%%%%end%%%%%%%%%%%%%%%%%%%%%%

%${\rm{3}}\frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + {\rm{3}}\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}\frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} \le \frac{{\partial ^{\rm{3}} {{\Pr}}_2^{\rm{e}} }}{{\partial ^{\rm{3}} r_{{\rm{RA}}} }}\frac{{\partial ^{\rm{3}} {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^{\rm{3}} r_{{\rm{RA}}} }}$

%So we have $2\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + {{\Pr}}_{{\rm{co}}}^{\rm{e}} \frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} + {{\Pr}}_2^{\rm{e}} \frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} > \frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} - \frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}$

%Hence$\frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{In}}} }}{{\partial r_{{\rm{RA}}} }} > \left| {\frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{De}}} }}{{\partial r_{{\rm{RA}}} }}} \right|$

%Hence we have the conclusion that: The mean of service rate ${\rm{E}}\left[ {s_i } \right]$ is first increasing and then decreasing in  $r_{{\rm{RA}}}$. 

Note that the overall  raw rate  $r_{{\rm{RA}}}$ is increasing in the overall error probability ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}$ and that the overall error probability ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}$ is increasing in the error probability  of the bottleneck link ${{{\Pr}}}^{{\rm{e}}} _i$, 
 we therefore have the following Proposition:

\noindent
\textbf {Proposition 4 } \emph {The BL-capacity ${\rm{E}}\left[ {s_i } \right]$ is first increasing and then decreasing in ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}$ or ${{{\Pr}}}^{{\rm{e}}} _i$. Thus, ${\rm{E}}\left[ {s_i } \right]$ has a unique maximum value.}
%

\
Proposition 4 shows that the BL-capacity of relaying is able to be maximized by choosing a proper target of ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}$ or ${{{\Pr}}}^{{\rm{e}}} _i$.


%\begin{equation}
%\frac{{\partial ^2 {\rm{E}}\left[ {s_i } \right]}}{{\partial ^2 r_{{\rm{RA}}} }} =  -
%2m\frac{{\partial {{\Pr}}_{{\rm{RA}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} - \frac{{\partial ^2 {{\Pr}}_{{\rm{RA}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}mr_{{\rm{RA}}} 
%\end{equation}





%\begin{equation}
%\begin{split}
% \frac{{\partial ^2 {{\Pr}}_{{\rm{RA}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} &= \frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}\left( {1 - {{\Pr}}_2^{\rm{e}} } \right) + \frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}\left( {1 - {{\Pr}}_{{\rm{co}}}^{\rm{e}} } \right) \\ 
%  &- 2\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} \\ 
% \end{split}
%\end{equation}


%We can learn that form Equation~\ref{eq:single_link_error_pro}:
%
%\begin{equation}
%\label{eq:single_link_error_derivative}
%\frac{{\partial {{\Pr}}_j^e }}{{\partial r}} = \sqrt {\frac{{2\pi m}}{{\left( {1 - 2^{ - 2c(x_j )} } \right)}}}  \cdot \frac{{e^{ - \frac{{m\left( {c(x_j ) - r} \right)^2 }}{{2\left( {1 - 2^{ - 2c(x_j )} } \right)\left( {\log _2 e} \right)^2 }}} }}{{\log _2 e}} > 0  \mathrm{,}
%\end{equation}
%
%\begin{equation}
%\label{eq:single_link_error_2derivative}
%\frac{{\partial ^2 {{\Pr}}_j^e }}{{\partial ^2 r}} = \frac{{m^{\frac{3}{2}} \sqrt {2\pi } \left( {c(x_j ) - r} \right)e^{ - \frac{{m\left( {c(x_j ) - r} \right)^2 }}{{2\left( {1 - 2^{ - 2c(x_j )} } \right)\left( {\log _2 e} \right)^2 }}} }}{{\left( {1 - 2^{ - 2c(x_j )} } \right)^{\frac{3}{2}} \left( {\log _2 e} \right)^3 }} \mathrm{.}
%\end{equation}

%Since the source determines the  raw rate  $r$ based on the perfect channel information, hence  raw rate  $r$ is smaller than the Shannon capacity of channel.
%Hence both $\frac{{\partial {{\Pr}}_j^e }}{{\partial r}}$ and $\frac{{\partial ^2 {{\Pr}}_j^e }}{{\partial ^2 r}} $ are positive.

%Then we divide the $\frac{{\partial {\rm{E}}\left[ {s_i } \right]}}{{\partial r_{{\rm{RA}}} }}$ into two parts:
%\begin{equation}
%\frac{{\partial {\rm{E}}\left[ {s_i } \right]}}{{\partial r_{{\rm{RA}}} }}={\mathop{\rm f}\nolimits} _{{\rm{In}}} \left( {r_{{\rm{RA}}} } \right) + {\mathop{\rm f}\nolimits} _{{\rm{De}}} \left( {r_{{\rm{RA}}} } \right)
%\end{equation}
%where ${\mathop{\rm f}\nolimits} _{{\rm{In}}} \left( {r_{{\rm{RA}}} } \right) $  and ${\mathop{\rm f}\nolimits} _{{\rm{De}}} \left( {r_{{\rm{RA}}} } \right)$ are the increasing part and decreasing part of the $\frac{{\partial {\rm{E}}\left[ {s_i } \right]}}{{\partial r_{{\rm{RA}}} }}$:
%\begin{equation}
%{\mathop{\rm f}\nolimits} _{{\rm{In}}} \left( {r_{{\rm{RA}}} } \right) = mr_{{\rm{RA}}} {{\Pr}}_{{\rm{co}}}^{\rm{e}} \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + mr_{{\rm{RA}}} \frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} {{\Pr}}_2^{\rm{e}} 
%\end{equation}
%\begin{equation}
%{\mathop{\rm f}\nolimits} _{{\rm{De}}} \left( {r_{{\rm{RA}}} } \right) = \left( {1 - {{\Pr}}_{{\rm{RA}}}^{\rm{e}} } \right)m - mr_{{\rm{RA}}} \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} - mr_{{\rm{RA}}} \frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}
%\end{equation}

%\begin{equation}
%\begin{array}{l}
% \frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{In}}} }}{{\partial r_{{\rm{RA}}} }} = m{\Pr} _{{\rm{co}}}^{\rm{e}} \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + m\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}{\Pr} _2^{\rm{e}}  \\ 
%  + mr_{{\rm{RA}}} \left( {2\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + {{\Pr}}_{{\rm{co}}}^{\rm{e}} \frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} + {{\Pr}}_2^{\rm{e}} \frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}} \right) \\ 
% \end{array}
%\end{equation}

%\begin{equation}
%\begin{array}{l}
% \frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{De}}} }}{{\partial r_{{\rm{RA}}} }} =  - 2m\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} - 2m\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + m{\Pr} _{{\rm{co}}}^{\rm{e}} \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + m{\Pr} _2^{\rm{e}} \frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} \\ 
%  - mr_{{\rm{RA}}} \left( {\frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} - \frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}} \right) \\ 
% \end{array}
%\end{equation}

%Then the 

%$\left\{ {2\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}} \right\}_{r_{{\rm{RA}}}  \to 0}  = \left\{ {\left( {1 - {{\Pr}}_{{\rm{co}}}^{\rm{e}} } \right)\frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} - \left( {1 - {{\Pr}}_2^{\rm{e}} } \right)\frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}} \right\}_{r_{{\rm{RA}}}  \to 0} $

%and

%${\rm{3}}\frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + {\rm{3}}\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}\frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} \le \frac{{\partial ^{\rm{3}} {{\Pr}}_2^{\rm{e}} }}{{\partial ^{\rm{3}} r_{{\rm{RA}}} }}\frac{{\partial ^{\rm{3}} {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^{\rm{3}} r_{{\rm{RA}}} }}$

%So we have $2\frac{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r_{{\rm{RA}}} }} + {{\Pr}}_{{\rm{co}}}^{\rm{e}} \frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} + {{\Pr}}_2^{\rm{e}} \frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} > \frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }} - \frac{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}{{\partial ^2 r_{{\rm{RA}}} }}$

%Hence$\frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{In}}} }}{{\partial r_{{\rm{RA}}} }} > \left| {\frac{{\partial {\mathop{\rm f}\nolimits} _{{\rm{De}}} }}{{\partial r_{{\rm{RA}}} }}} \right|$

%Hence we have the conclusion that: The mean of service rate ${\rm{E}}\left[ {s_i } \right]$ is first increasing and then decreasing in  $r_{{\rm{RA}}}$. Note that the $r_{{\rm{RA}}}$ is the increasing function of the target overall error probability, therefore we have the follow Proposition:

%\noindent
%\textbf {Proposition 4 } \emph {The mean of service rate ${\rm{E}}\left[ {s_i } \right]$ is first increasing and then decreasing in the overall error probability ${{{\Pr}}}^{{\rm{e}}} _{\rm{RA}}$.}


% 我们需要证明 overall probability 是 单调递增函数

%The $ r({\bf{h}}_1^2   + {\bf{h}}_3^2  , {{{\Pr}}}^{{\rm{e}}}_3 )$ has the following properties:
%\begin{itemize}
%  \item  $ r({\bf{h}}_1^2   + {\bf{h}}_3^2  , {{{\Pr}}}^{{\rm{e}}}_3 )$
%\end{equation}


%$1 slot = 0.5ms = 1/2000 s$

% m $=$ 200 to 600 means the $T_f =$ 0.1s to 0.3s .

==> v 2.7_single_black/4_MSDR.tex <==
%\section{The system performance for fading channel}
\section{The BL-capacity with Fading Channels}
\label{sec:Effective_Rate_Block_Fading}
%
%\begin{equation}
%s_i  = \left\{ {\begin{array}{*{20}c}
%   {m\bar r(\alpha _1  + {\rm{h}}_3^2  )} & {with\;prob.\;\left[ {1 - \varepsilon (\alpha _2 )} \right] \cdot \left[ {1 - \varepsilon (\alpha _1  + {\rm{h}}_3^2  )} \right]}   \\
%   {m\bar r(\alpha _1 )} & {with\;prob.\;\varepsilon (\alpha _2 )\left[ {1 - \varepsilon (\alpha _1 )} \right]}   \\
%   0 & { 
%{with\;prob.\left[ {1 - \varepsilon (\alpha _2 )} \right]\varepsilon (\alpha _1  + {\rm{h}}_3^2  ) + \varepsilon (\alpha _2 )\varepsilon (\alpha _1 )}}   \\
%\end{array}} \right.
%\end{equation}
In this section,  we extend the  results of Section~\ref{sec:Effective_Rate_relay} to block-fading channels where the channel gains remain constant within a frame (two phases) and vary from one frame to the next. In other words, the channels are fixed  within every single two-phases transmission of a packet. %Therefore, the analysis of relaying performance with non-fading channels are still valid in each single frame of block-fading channels.% of the fading channels. 


%\subsection{Maximize the expected value of BL-capacity per frame} 

As the CSI of all the links are available at the source, %Based on our analysis in Section~\ref{sec:Effective_Rate_relay},
 the source is required to determine the value of overall  raw rate  $ r_{\rm{RA}} $ to maximize  the BL-capacity (the expected value of the service process) in each  frame. 
%Therefore, with the block-fading channels the source is able to  maximize the expected value of BL-capacity for each frame.
 As a result, the overall  raw rate  is varying along with the channel fading from frame to frame and can be denoted by $r _{{\rm{RA}},i}$ where $i$ is the index of frames.  Therefore, the service process $s_i$ under a block-fading channel assumption can be modeled as (in bits per m channel use):
\begin{equation}
s_i  =2m\phi_i r _{{\rm{RA}},i}\mathrm{,}
\end{equation}
where $\phi_i  $ is a binary random variable defined by   $\Pr \{ \phi_i  = 1\}  = {1\! -\!  {{\Pr}}^{{\rm{e}}} _{{\rm{RA}},i}  }$, $\Pr \{ \phi_i  = 0\}  = { {{\Pr}}^{{\rm{e}}} _{{\rm{RA}},i}  }$ and $r_{{\rm{RA}},i}$ is chosen by maximizing the expected value of $s_i$ for frame $i$.
%
Finally, the BL-capacity  over frames therefore can be obtained by the sample mean of the service process: %\footnote{The equation  presented in~\eqref{eq:mean__} is the mean of the service process. , the derivation of it will be presented in our future work.}:
${\rm{E}}\left[ {{s_i}} \right] = \mathop {\lim }\limits_{I \to  + \infty } \frac{{\sum\nolimits_{i = 1}^I {\left( {1 - \Pr _{{\rm{RA}},i}^{\rm{e}}} \right) \cdot 2m{r_{{\rm{RA}},i}}} }}{I}$. % = 2m \iint {\left( {1 - \Pr _{{\rm{RA}},i}^{\rm{e}}} \right) \cdot {r_{{\rm{RA}},i}}}d{x_{\rm{co}}}d{x_2}$
%\begin{equation}
% {\mathop{\rm E} } \left[ {s_i } \right] = \sum\nolimits_{i = 1}^{ + \infty } {\left( {1 - {\Pr}_{{\rm{RA,}}i}^{\rm{e}} } \right) \cdot %2mr_{{\rm{RA},}i}} 
%\; \mathrm{.}
%\label{eq:mean__}
%\end{equation}
%where the ${{\mathop{\rm E}\limits_z} \left[ {s_i } \right]} $ the expected value of $s_i$ over channel fading while $z$ denotes channel gain variable.

%In addition, the variance of the service rate $s_i$ can be obtained by:
%\begin{equation}
%\begin{split}
% {\mathop{\rm Var}\nolimits} \left[ {s_i } \right] = &\sum\nolimits_{i = 1}^{ + \infty } { { {\Pr}_{{\rm{RA,}}i}^{\rm{e}} {\mathop{\rm E}\nolimits} \left[ {s_i } \right]^2 } }  \\ 
%  + &\sum\nolimits_{i = 1}^{ + \infty } { {\left( {1 - {\Pr}_{{\rm{RA,}}i}^{\rm{e}} } \right)\left( {2mr_{{\rm{RA,}}i}  - {\mathop{\rm E}\nolimits} \left[ {s_i } \right]} \right)^2 }}  \\ 
% \end{split}
%\end{equation}


%\input{fixed_error_probability}

%\begin{equation}
%\begin{array}{l}
% \left( {c_1  + c_2 \cdot Q^{ - 1} \left( {\Pr _j^{\rm{e}} } \right)} \right) \\
% \left\{ \begin{array}{l}
% {{\Pr}}_2^{\rm{e}} \left( {\frac{{\partial ^2 {{\Pr}}_1^{\rm{e}} }}{{\partial ^2 r}}\left( {\frac{{\partial r}}{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}} \right)^2  + \frac{{\partial {{\Pr}}_1^{\rm{e}} }}{{\partial {\rm{r}}}}\frac{{\partial ^2 r}}{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}} \right) \\ 
%  + \left\{ {2\frac{{\partial {{\Pr}}_1^{\rm{e}} }}{{\partial r}}\frac{{\partial r}}{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }} - {\rm{1}}} \right\}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r}}\frac{{\partial r}}{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }} \\ 
%  + \left\{ {{{\Pr}}_1^{\rm{e}}  - {{\Pr}}_{{\rm{co}}}^{\rm{e}}  - 1} \right\}\left( {\frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r}}\left( {\frac{{\partial r}}{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}} \right)^2  + \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r}}\frac{{\partial ^2 r}}{{\partial ^2 {{\Pr}}_{{\rm{co}}}^{\rm{e}} }}} \right) \\ 
% \end{array} \right\} \\ 
%  > c_2 \left\{ \begin{array}{l}
% \left( {1 - {\Pr}_{{\rm{RA}}}^{\rm{e}} } \right) \cdot 2\pi Q^{ - 1} \left( {\Pr _j^{\rm{e}} } \right)e^{\left( {Q^{ - 1} \left( {\Pr _j^{\rm{e}} } \right)} \right)^2 }  \\ 
% \left\{ {{{\Pr}}_1^{\rm{e}}  - {{\Pr}}_{{\rm{co}}}^{\rm{e}} } \right\}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r}}\frac{{\partial r}}{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }} \cdot 2\sqrt {2\pi } e^{\frac{{\left( {Q^{ - 1} \left( {\Pr _j^{\rm{e}} } \right)} \right)^2 }}{2}}  \\ 
% \left\{ {{{\Pr}}_2^{\rm{e}} \frac{{\partial {{\Pr}}_1^{\rm{e}} }}{{\partial r}}\frac{{\partial r}}{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }} + 1 - {{\Pr}}_2^{\rm{e}} } \right\}2\sqrt {2\pi } e^{\frac{{\left( {Q^{ - 1} \left( {\Pr _j^{\rm{e}} } \right)} \right)^2 }}{2}}  \\ 
% \end{array} \right\} \\ 
% \end{array}
%\end{equation}

%What we need to prove:
%\begin{equation}
%\begin{array}{l}
% \frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r}}\left( {c_1  + c_2 Q^{ - 1} \left( {\Pr _j^{\rm{e}} } \right)} \right) + \sqrt {2\pi } {{\Pr}}_2^{\rm{e}} \left( {c_1  + c_2 Q^{ - 1} \left( {\Pr _j^{\rm{e}} } \right)} \right)e^{\frac{{\left( {Q^{ - 1} \left( {\Pr _{{\rm{co}}}^{\rm{e}} } \right)} \right)^2 }}{2}}  \\ 
% \left\{ \begin{array}{l}
% \left( {\frac{{\partial ^2 {{\Pr}}_1^{\rm{e}} }}{{\partial ^2 r}} - \left( {1 + {{\Pr}}_{{\rm{co}}}^{\rm{e}}  - {{\Pr}}_1^{\rm{e}} } \right)\frac{{\partial ^2 {{\Pr}}_2^{\rm{e}} }}{{\partial ^2 r}}} \right)c_2  +  \\ 
% \left( {\frac{{\partial {{\Pr}}_1^{\rm{e}} }}{{\partial {\rm{r}}}} - \left( {1 + {{\Pr}}_{{\rm{co}}}^{\rm{e}}  - {{\Pr}}_1^{\rm{e}} } \right)\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r}}} \right)Q^{ - 1} \left( {\Pr _{{\rm{co}}}^{\rm{e}} } \right) \\ 
%  + 2c_2 \frac{{\partial {{\Pr}}_1^{\rm{e}} }}{{\partial r}}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r}} \\ 
% \end{array} \right\} \\ 
%  > \left\{ \begin{array}{l}
% \left( {1 - {\Pr}_{{\rm{RA}}}^{\rm{e}} } \right) \cdot \sqrt {2\pi } Q^{ - 1} \left( {\Pr _j^{\rm{e}} } \right)e^{\frac{{\left( {Q^{ - 1} \left( {\Pr _{{\rm{co}}}^{\rm{e}} } \right)} \right)^2 }}{2}}  \\ 
% 2\left\{ {{{\Pr}}_1^{\rm{e}}  - {{\Pr}}_{{\rm{co}}}^{\rm{e}} } \right\}\frac{{\partial {{\Pr}}_2^{\rm{e}} }}{{\partial r}}\frac{{\partial r}}{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }} \\ 
% 2\left\{ {{{\Pr}}_2^{\rm{e}} \frac{{\partial {{\Pr}}_1^{\rm{e}} }}{{\partial r}}\frac{{\partial r}}{{\partial {{\Pr}}_{{\rm{co}}}^{\rm{e}} }} + 1 - {{\Pr}}_2^{\rm{e}} } \right\} \\ 
% \end{array} \right\} \\ 
% \end{array}
%\end{equation}



%\begin{equation}
%\frac{{\partial {{\Pr}}_j^{\rm{e}} }}{{\partial r}} = \frac{1}{{\sqrt {2\pi } }}\exp \frac{m}{2}\frac{{\left[ {\log \left( {1 + \frac{{z_j p_{{\rm{tx}}} }}{{\sigma ^2 }}} \right) - r} \right]^2 }}{{\left( {1 - \left( {1 + \frac{{z_j p_{{\rm{tx}}} }}{{\sigma ^2 }}} \right)^{ - 2} } \right)\left( {\log _2 e} \right)^2 }}
%\end{equation}

%\begin{equation}
%\frac{{\partial ^2 {{\Pr}}_j^{\rm{e}} }}{{\partial ^2 r}} = \frac{m}{{2\sqrt {2\pi } }}\frac{{\left[ {r - \log \left( {1 + \frac{{z_j p_{{\rm{tx}}} }}{{\sigma ^2 }}} \right)} \right]e^{\frac{m}{2}\frac{{\left[ {\log \left( {1 + \frac{{z_j p_{{\rm{tx}}} }}{{\sigma ^2 }}} \right) - r} \right]^2 }}{{\left( {1 - \left( {1 + \frac{{z_j p_{{\rm{tx}}} }}{{\sigma ^2 }}} \right)^{ - 2} } \right)\left( {\log _2 e} \right)^2 }}} }}{{\left( {1 - \left( {1 + \frac{{z_j p_{{\rm{tx}}} }}{{\sigma ^2 }}} \right)^{ - 2} } \right)\left( {\log _2 e} \right)^2 }}
%\end{equation}

%As proved in~\cite{Gursoy_2011} the average transmission rate over a (one hop) single link is a  concave function of the error probability of this link. Hence, the average transmission rate of the bottleneck link is a concave function of its error probability. In addition, as analyzed in \textbf {Proposition 2}, ${\rm{\Pr}}_{{\rm{RA}}}^e$ is the a increasing function of  ${\rm{\Pr}}_{j}^e$. It also can be proved that $\frac{{1 - \hat {\rm{\Pr}}_{{\rm{RA}}}^e ({\rm{\Pr}} _j^e )}}{{1 - {\rm{\Pr}} _j^e }}$ is increasing in ${\rm{\Pr}} _j^e$.
 


%Therefore the ${\rm{E}}\left[ {s_i } \right]$ can be expressed the as a product of a increasing function $incr({\rm{\Pr}} _{j}^{e})$ and a concave function $conc({\rm{\Pr}} _{j}^{e})$:
%\begin{equation}
%\begin{split}
%{\mathop{\rm E}\nolimits} \left[ {s_i } \right] &= incr({\rm{\Pr}} _{j}^{e}) \cdot  conc({\rm{\Pr}} _{j}^{e}) \\
%&= \frac{{(1 - \hat {\rm{\Pr}}_{{\rm{RA}}}^e )}}{{(1 - {\rm{\Pr}} _j^e )}} \cdot m(1 - {\rm{\Pr}} _{j}^{e} ){\mathop{\rm E}\nolimits} \left[ {r_{{\rm{RA}}} } ({\rm{\Pr}} _{j}^{e})\right]\\
%\end{split}
%\end{equation}

%\begin{proof}
%\textbf {the proof has not been finished}

%$\because$ the follow reasons:
%\begin{itemize}
%\item $conc({\rm{\Pr}} _{j}^{e})$ is first increasing and then decreasing in ${\rm{\Pr}} _{j}^{e}$.
%\item $incr({\rm{\Pr}} _{j}^{e})$ is increasing in ${\rm{\Pr}} _{j}^{e}$.
%\item both  $conc({\rm{\Pr}} _{j}^{e})$ and $incr({\rm{\Pr}} _{j}^{e})$  are positive.
%\end{itemize}
%$\therefore$ we have the follow conclusion:
%\begin{itemize}
%\item if    $\left. {\frac{{\partial {\rm{E}}\left[ {s_i } \right]}}{{\partial {\rm{\Pr}} _j^e }}} \right|_{{\rm{\Pr}} _j^e  \to 1}  \ge 0$   then the  ${\rm{E}}\left[ {s_i } \right]$ is increasing in ${\Pr} _{j}^{e}$.
%\item if   $\left. {\frac{{\partial {\rm{E}}\left[ {s_i } \right]}}{{\partial {\rm{\Pr}} _j^e }}} \right|_{{\rm{\Pr}} _j^e  \to 1}  < 0$    then the  ${\rm{E}}\left[ {s_i } \right]$ is first increasing and then decreasing in ${\rm{\Pr}} _{j}^{e}$.
%\end{itemize}

%\end{proof}
%
%Hence, the MSDR of the system (per m channel use) can be given as:
%\begin{equation}
%\left. {R } \right|_{\left\{ {d,P_d } \right\}}  \approx \frac{{{m \bar r_O}\left( {1 - \varepsilon _{\rm{O}} } \right)}}{2}\left( {1 + \sqrt {1 + \frac{{2\varepsilon _{\rm{O}} \ln \left( {P_d } \right)}}{{d\left( {1 - \varepsilon _{\rm{O}} } \right)}}} } \right) \mathrm{,}
%\label{eqn:effective_rate_final}
%\end{equation}
%and the normalized MSDR in bits per channel use is given as:
%\begin{equation}
%\left. {\bar R} \right|_{\left\{ {d,P_d } \right\}}\! =\! \frac{{\left. R \right|_{\left\{ {d,P_d } \right\}} }}{m} \! \approx \! \frac{{{ \bar r_O}\left( {1 \!-\! \varepsilon _{\rm{O}} } \right)}}{2}\left( {1 \!+\! \sqrt {1 \!+\! \frac{{2\varepsilon _{\rm{O}} \ln \left( {P_d } \right)}}{{d\left( {1 \!-\! \varepsilon _{\rm{O}} } \right)}}} } \right) \mathrm{.}
%\label{eqn:effective_rate_final}
%\end{equation}
%\noindent
%\textbf {Proposition 4 (miss proof)} \emph {For a given QoS requirement pair $\{d, P_d\}$, the maximum sustainable data rate is first increasing and later decreasing on overall error probability~$\bar \varepsilon_{\rm{O}}$.}%, and also a convex function of the bottleneck link error probability $\varepsilon_i$.}
%








==> v 2.7_single_black/5_simulation.tex <==
%\newpage
\section{NUMERICAL RESULTS AND DISCUSSION}
\label{sec:simulation}


In this section, we first show the appropriateness of our theoretical model. Subsequently, we evaluate the performance of the studied relaying system (with average CSI) in comparison to direct transmission and relaying with perfect CSI. 

For the numerical results, we consider the following parameterization of the system model:
 {{First of all, we consider the cases with blocklength $m \ge 100$  (at each hop of relaying), for
which the approximation is tight enough\footnote{{{The choice of $m \ge 100$ as the minimum
possible length is motivated by [10, Fig. 2] where the relative
difference of the approximate  and the exact achievable rates is
less than 2\% for the cases with $m \ge$ 100.}}}.
In addition, the codewords length of each link is set to be the same as the blocklength.}}
Secondly,  we consider an outdoor urban scenario and the  distances of the backhaul, relaying and direct links are set to 200~$\rm{m}$, 200~$\rm{m}$ and 360~$\rm{m}$. Thirdly, we set the transmit power $p_{\rm{tx}}$  equal to 30~$\rm{dBm}$ and noise power to -90~$\rm{dBm}$,  respectively.  
In addition, we utilize the well-known COST~\cite{Molisch_2011} model for calculating the path-loss while the center frequency is set to equal  2~$\rm{GHz}$. Regarding the channel,  we only consider quasi-static channel model in the simulation.  Hence, the numerical results for all validations and evaluations are based on the average/ergodic performance over the random channel fading. 
Moreover,  as we consider the {{link}}-layer performance, in the simulation the QoS constraints \{delay, delay violation probability\} are set to $\{10^{4}$~symbols, $10^{-2}\}$.  
Finally, to observe the relaying performance we mainly vary the following parameters in the simulation: Blocklength and weight factor~$\eta$.



%Without channel information at transmitters, the system has lower performance than with perfect CSI. This can be learned by comparing the MSDRs in Figure~\ref{MSDR_withoutCSI} to the MSDRs in the previous Figures.  It should be mentioned that the gap between lower bound and higher bound is significant with short blocklength.



\subsection{Appropriateness of our theoretical model}

In Figure~\ref{Capacity_codingratewithoutCSI} we show the relationship between the relaying performance and the coding rate. We plot the related (ergodic) Shannon capacity of relaying as a reference. As shown in the figure, the Shannon capacity is not influenced by the coding rate. 
More importantly,  it is shown that the BL-throughput and the MSDR are concave in  the coding rate, which matches Theorem  1 and 2.
During the low coding rate region, both the BL-throughput and the MSDR increase approximately linearly as the coding rate increases.  This is due to the fact that  errors hardly occur with a low coding rate. Hence, the bottleneck of the performance is the coding rate. However, as the coding rate continues increasing, the error probability becomes  more and more significant. As a result, the error probability then becomes the major limit of the system performance.   Therefore, both  the BL-throughput and the MSDR  decrease during the higher coding rate region.
%The related overall probability is show in Figure~\ref{overall_error_probability_withoutCSI}. 
\begin{figure}[!h]
\begin{center}
\includegraphics[width=0.55\linewidth, trim=10 20 10 0 ]{Capacity_codingrate.pdf}
\end{center}
\caption{The performance of the studied relaying system (average CSI at the source).}
\label{Capacity_codingratewithoutCSI}
\end{figure}







\begin{figure}[!h]
\begin{center}
\includegraphics[width=0.55\linewidth, trim=10 15 10 0 ]{Capacity_weight.pdf}
\end{center}
\caption{The relaying performance versus the weight factor.}
\label{capacityvs_weight}
\end{figure}

Figure~\ref{capacityvs_weight} validates  Corollary 1 and 2 that both  the BL-throughput and the MSDR are quasi-concave in the weight factor $\eta$.
Hence,  the weight factor introduces a good tradeoff between the coding rate and the error probability to the studied relaying system (only with average CSI at the source). Based on this tradeoff, both the physical-layer performance and the {{link}-layer performance of the system can be optimized. Moreover, it  can also be observed from Figure~\ref{capacityvs_weight}  that the optimal values of the weight factor for maximizing the BL-throughput and for maximizing the MSDR are not the same. 
Moreover, we also find in the simulation (not shown here) that the optimal $\eta$ for maximizing the MSDR is subject to the QoS constraints. In particular, the stricter the constraints are the smaller the optimal $\eta$ is.
Hence, the parameterization of  the weight factor $\eta$ for a QoS-support system and a non-QoS-support system should be treated differently. 
These are important guidelines for the design of the studied relaying system.  



In Figure~\ref{weightfactorwork}, we provide intuitive parallel sub-figures  to show how the weight factor introduces the tradeoff between the coding rate and the error probability and further influences the BL-throughput and the MSDR.
%
\begin{figure}[!h]
\begin{center}
\includegraphics[width=0.55\linewidth, trim=10 15 10 20 ]{weight_process.pdf}
\end{center}
\caption{How the weight factor introduces tradeoff between error probability and coding rate and further influences the BL-throughput and the MSDR?   In the simulation, the blocklength at each hop of relaying is 500 symbols.}
\label{weightfactorwork}
\end{figure}
%
As shown in the figure, by increasing the weight factor the coding rate increases as well as the error probability.  In particular, the coding rate increases rapidly at the beginning but slowly later on. At the same time, the error probability increases approximately linearly. 
As a result, the BL-throughput/MSDR first increases and then deceases. In other words, they are quasi-concave in the weight factor  $\eta$.



\subsection{Evaluation}
So far, we have shown the appropriateness of our Theorems and corollaries. 
In the following, we further evaluate the studied relaying system. {{{In the evaluation, the performance under the perfect CSI scenario is considered as a contrast. In particular, a result of the (average) BL-throughput with the perfect CSI is obtained by maximizing the instantaneous BL-throughput\footnote{{{In~[15] we show that the BL-throughput of relaying can be maximized by choosing an appropriate coding rate $r$ (based on the perfect CSI) for AWGN channels. This also holds for maximizing the instantaneous BL-throughput at each transmission period under the  quasi-static channels.}}} for each transmission period based on the perfect CSI.}}}

\subsubsection{Under average CSI scenario: relaying performance vs. blocklength}
We first show the relationship between the performance of the studied relaying system and the blocklength in Figure~\ref{capacity_blocklength}. The figure shows that the BL-throughput of the studied relaying system is slightly increasing in the blocklength while the MSDR is significantly decreasing in the blocklength. The explanation is as follows. 
%
\begin{figure}[!h]
\begin{center}
\includegraphics[width=0.55\linewidth, trim=10 15 -0 10 ]{capacity_blocklength.pdf}
\end{center}
\caption{The relaying performance versus blocklength.}
\label{capacity_blocklength}
\end{figure}
%
On one hand, based on~\eqref{eq:single_link_error_pro} and~\eqref{eq:single_link_data_rate} both error probability and coding rate are influenced by the blocklength $m$. In particular, with a fixed coding rate at each link a long blocklength leads to a low error probability of each link. Obviously, this results in a low overall error probability of relaying and therefore a high BL-throughput. This is the reason why the BL-throughput is slightly increasing in the blocklength. On the other hand, a long blocklength means that a single transmission (i.e., two-hop relaying) costs a long time. This reduces the number of allowed retransmission attempts under a given delay constraint. For example, consider a relaying system where the blocklength of each hop of relaying is $500$ symbols (two-hop relaying transmission period is $10^{3}$ symbols). 
To support a service with a delay constraint $d = 10^{4}$ symbols,  the maximal number of transmission attempts (including an initial transmission and retransmissions),  which not violates the delay constraint, is 10  times.  This number would be 5 if the blocklength is doubled. In other words, a long blocklength reduces the flexibility of a QoS-support system due to limiting the number of transmission attempts.     At the same time, the gain from increasing blocklength becomes tiny as the blocklength increases (e.g., even ragarding the physical-layer performance, the BL-throughput is approximately a constant during the long blocklength region).   As a result, the MSDR reduces significantly in the long blocklength region. For an extreme example, the MSDR is zero if the blocklength is longer than the delay constraint. 

%It should be mentioned that the above observation "MSDR is concave in the blocklength" is an important guideline for determining the blocklength in the design of QoS-support relaying systems.






\subsubsection{Under average CSI scenario: relaying vs. direct transmission --- observing the performance advantage of relaying}

Under the average CSI scenario, we compare the  performance of the studied relaying system with  direct transmission.
%
%Next, we compare the  performance of the studied relaying system (with average CSI) with  direct transmission as well as  relaying with perfect CSI.
To make a fair comparison, we set the coding rate of direct transmission to be equal to the equivalent coding rate of relaying.  In addition, we set the blocklength of direct transmission to be twice  as large as the blocklength at each hop of relaying. Hence, the length of each transmission period of relaying equals that of direct transmission.  % More importantly, we adjust the relay location to 
%
%
\begin{figure}[!h]
\begin{center}
\includegraphics[width=0.55\linewidth, trim=10 18 10 7 ]{averageCSIvsNorelaying_factor.pdf}
\end{center}
\caption{The performance comparison between relaying (with average CSI) and direct transmission (with average CSI) while varying the weight factor $\eta$.   In the simulation, the blocklength at each hop of relaying is 500 symbols. }
\label{Relayingvsderct_codingrate}
\end{figure}
%
%
\begin{figure}[!h]
\begin{center}
\includegraphics[width=0.55\linewidth, trim=10 18 -15 10 ]{averageCSIvsNorelaying_blocklength.pdf}
\end{center}
\caption{The performance comparison between relaying (with average CSI) and direct transmission (with average CSI) under dynamic blocklength ($\eta=0.2$).}
\label{Relayingvsderct_blocklength}
\end{figure}
%
Under the above setup, we compare the two schemes in Figure~\ref{Relayingvsderct_codingrate} and Figure~\ref{Relayingvsderct_blocklength}
where we vary the coding rate and blocklength, respectively.
Based on these two figures, we observe that {{both the BL-throughput and the MSDR of relaying significantly outperform direct transmission}},  although these two schemes have a similar Shannon capacity.  
In other words, under the average CSI scenario relaying shows a significant advantage (in comparison to the direct transmission)  on the blocklength-limited performance.  

\subsubsection{The performance advantage of relaying: under perfect CSI scenario vs. under average CSI scenario}
The previous subsection shows the performance advantage of relaying  under the average CSI scenario. In this subsection, we compare this performance advantage under the  average CSI scenario with the one under the perfect CSI scenario. 
We show the comparison in  Figure~\ref{averageCSI_vs_perfectCSI_weight} and Figure~\ref{averageCSI_vs_perfectCSI_blocklength} where the weight factor and the blocklength are varied respectively.
\begin{figure}[!h]
\begin{center}
\includegraphics[width=0.55\linewidth, trim=10 12 10 15 ]{averageCSI_vs_perfectCSI_weight.pdf}
\end{center}
\caption{The performance comparison between relaying with average CSI and relaying with perfect CSI while varying the weight factor ($\eta=0.2$).}
\label{averageCSI_vs_perfectCSI_weight}
\end{figure}
%
%
\begin{figure}[!h]
\begin{center}
\includegraphics[width=0.55\linewidth, trim= 10 19 10 12 ]{averageCSI_vs_perfectCSI_blocklength.pdf}
\end{center}
\caption{The performance comparison between relaying with average CSI and relaying with perfect CSI under dynamic blocklength ($\eta=0.2$).}
\label{averageCSI_vs_perfectCSI_blocklength}
\end{figure}
In general, these figures show that relaying has better blocklength-limited performance than direct transmission under both the perfect CSI scenario and the  average CSI scenario. %This is the performance advantage of relaying under the finite blocklength regime (in comparison to the Shannon capacity regime), which has been first observed in~\cite{Hu_2015} under the perfect CSI scenario. 
However, we further observe that this performance advantage of relaying under the average CSI scenario is more significant than under the perfect CSI scenario, i.e.,  the performance improvement by relaying {{(comparing relaying with direct transmission)}} under the  average CSI scenario  is significantly higher than the one under the perfect CSI scenario. 
{{{Recall that in~\cite{Hu_2015} we have shown that  with perfect CSI relaying is more beneficial  {in}  the finite blocklength regime in comparison to  {in}  the Shannon capacity regime.
 The observation from Figure~\ref{averageCSI_vs_perfectCSI_weight} and Figure~\ref{averageCSI_vs_perfectCSI_blocklength} further indicates that}}}  in  the finite blocklength regime  relaying is more beneficial for the average CSI scenario in comparison to the  perfect CSI scenario.  This is another important guideline for the design of blocklength-limited systems.






\subsubsection{The performance loss due to a finite blocklength: under perfect CSI scenario vs. under average CSI scenario}


Finally, we compare the performance losses due to a finite blocklength under perfect CSI scenario and under average CSI scenario. 
 {{Under the perfect CSI scenario, the performance loss due to a finite blocklength is actually the performance gap between the Shannon capacity and the BL-throughput (with perfect CSI).
On the other hand, this performance loss under the average CSI scenario is observed by comparing the BL-throughput (with average CSI) with the outage capacity.}} 
 In particular,  the  outage capacity  is a performance metric  {in}  the Shannon capacity regime. % for the imperfect CSI scenario.
  It is given by $r \left( {1 - {{\Pr }_{{\rm{out}}}}(r )} \right)$, where~${{{\Pr }_{{\rm{out}}}}(r )}$ is the outage probability.
To calculate the outage capacity, the weighting CSI operation is also considered in the simulation, i.e., the packet size is chosen based on the Shannon capacity  of the weighted CSI. %Moreover, in the simulation we set theses different scenarios have the same frame length which equals the blocklength of each hop of relaying.

%
\begin{figure}[!h]
\begin{center}
\includegraphics[width=0.55\linewidth, trim=20 35 10 10 ]{averageCSI_perfectCSI_FB_vs_Shannon_relaying_less.pdf}
\end{center}
\caption{The performance comparison between relaying  {in}  the Shannon capacity regime and relaying  {in}  the finite blocklength regime (blocklength at each hop of relaying is 500 symbols).}
\label{fbRelaying_vs_Shannonrelaying}
\end{figure}
%
Under the above setup, we first show the numerical results of the comparison in Figure~\ref{fbRelaying_vs_Shannonrelaying} where we fix the blocklength and vary the weight factor. 
The figure shows that the  performance loss due to a finite blocklength is considerable under the perfect CSI scenario. 
However, we find that under the average CSI scenario the performance loss due to a finite blocklength is negligible. 
In the simulation, we also observe that (not shown here)  only with average CSI at the source the outage probability ({in}  the Shannon capacity regime) and the average error probability ({in}  the finite blocklength regime) have similar performance. 

The observations from Figure~\ref{fbRelaying_vs_Shannonrelaying} are based on the   setup that the blocklength equals $m=500$ symbols.
Recall that the BL-throughput is limited by the blocklength and the performance  {in}  the Shannon capacity regime is not influenced by the blocklength. Hence, the performance loss due to a finite blocklength should also be subject to the blocklength. 
Then, we further investigate this performance loss in Figure~\ref{fbRelaying_vs_Shannonrelaying_vary_m} where we vary the blocklength.
%
\begin{figure}[!h]
\begin{center}
\includegraphics[width=0.55\linewidth, trim=10 15 10 10 ]{averageCSI_perfectCSI_FB_vs_Shannon_relaying_less_vary_m.pdf}
\end{center}
\caption{The performance comparison between relaying  {in}  the Shannon capacity regime and relaying  {in}  the finite blocklength regime while varying the blocklength. In the simulation, $\eta=0.2$.}
\label{fbRelaying_vs_Shannonrelaying_vary_m}
\end{figure}
%
Again, we observe  that the performance loss under the average CSI scenario is much smaller than the one under the perfect CSI scenario.  In particular, with a non-extremely short blocklength (e.g., blocklength $m >100$) the performance loss due to a finite blocklength  is negligible under the average CSI scenario. 


From Figure~\ref{fbRelaying_vs_Shannonrelaying_vary_m} we observe that the BL-throughput of relaying with average CSI and the outage capacity converge quickly.   It should be mentioned that this is not a unique characteristic of relaying. It is studied and observed in~\cite{Yang_2014} that  the  speed of convergence between the BL-throughput and the outage capacity for a non-relaying direct transmission is also fast. This motivates us to compare the speeds of convergence of these two transmissions schemes. We show the comparison in Figure~\ref{Thelastone}.
\begin{figure}[!h] 
\begin{center}
\includegraphics[width=0.55\linewidth, trim=20 15 0 10 ]{lastone.pdf}
\end{center}
\caption{The speed of convergence between the BL-throughput with average CSI and  the outage capacity. }
\label{Thelastone}
\end{figure}
From the figure, we first observe that relaying has a slightly faster speed of convergence in comparison to direct transmission. In addition, in general both these two schemes  have quick speeds of convergence between the BL-throughput with average CSI and the outage capacity. This  observation is different from the case with perfect CSI shown in Figure~\ref{averageCSI_vs_perfectCSI_blocklength} where  speeds of the convergence (between the BL-throughput and the Shannon capacity) for both relaying and direct transmission are relatively slow. More interesting,  Figure~\ref{averageCSI_vs_perfectCSI_blocklength} shows that  the speed of convergence  of relaying is also faster than direct transmission under the  perfect CSI scenario. Combining Figure~\ref{averageCSI_vs_perfectCSI_blocklength}   and Figure~\ref{Thelastone}, we conclude that (although halving the blocklength) relaying surprisingly has a  faster  speed of convergence (between the blocklength-limited performance and the performance in the Shannon capacity regime) in comparison to direct transmission under both the average CSI scenario and the perfect CSI scenario. {{{This is actually the performance advantage of relaying  in the finite blocklength regime from a perspective of the speed of convergence (to the Shanon/outage capacity).}}}
% It should be mentioned that the fast speed of convergence between the BL-throughput and the outage capacity for a non-relaying direct transmission was firstly studied and observed in~\cite{Yang_2014}. Our work takes this one  step further in a relaying network and shows that although halving the blocklength relaying has a more faster  speed of convergence.}}





==> v 2.7_single_black/7_Conclusion.tex <==
\section{Conclusion}
\label{sec:Conclusion}


Under the finite blocklength regime, we investigated the  physical-layer performance (BL-throughput) as well as the {{link}}-layer performance (MSDR) of a relaying system with quasi-static fading channels but only the average CSI (at the source). 
%In this work,  we focused on the blocklength-limited performance of a relaying system where quasi-static fading channels are considered while  only the average CSI is assumed to be available at the source.  Both the physical-layer performance (BL-throughput) and the higher-layer performance (effective capacity) of the system were  investigated. 
We proposed a simple system operation by introducing a factor based on which we weight the average CSI and let the source determine the coding rate based on the weighted CSI. The BL-throughput  and the MSDR of the studied relaying system are investigated.  
Moreover, we proved that both the  BL-throughput and the MSDR are  concave in the coding rate.
More importantly, it was proved that the  BL-throughput and the MSDR are  quasi-concave in the weight factor. In other words, the performance of the studied system can be easily optimized based on the proposed operation.

We concluded a set of guidelines for the design of efficient relaying systems (under the finite blocklength regime) from numerical analysis.
Firstly, under the average CSI scenario the BL-throughput of relaying is slightly increasing in the blocklength while the effective capacity is significantly decreasing in the blocklength. Hence, determining the blocklength is very important for the design of QoS-support relaying systems. 
Secondly, the weight factor we proposed introduces a good tradeoff between the coding rate and the error probability to the studied relaying system. Based on this tradeoff, both the physical-layer performance and the {{link}}-layer performance of the system can be optimized. Moreover, the optimal values of the weight factor for maximizing the BL-throughput and for maximizing the MSDR are  different.  
Thirdly, under the condition of having similar Shannon capacity performance relaying outperforms direct transmission in the finite blocklength regime. This is actually the performance advantage of relaying in the  finite blocklength regime. 
More importantly,  this performance advantage of relaying under the average CSI scenario is more significant than under the perfect CSI scenario. 
In addition,  the performance loss due to a finite blocklength (i.e., the performance gap between the performance in the Shannon capacity regime and in the finite blocklength regime) is negligible under the average CSI scenario in comparison to the one under the perfect CSI scenario. {{Moreover, the speed of convergence (between the blocklength-limited performance and the performance in the Shannon capacity regime) in relaying system is faster in comparison to the direct transmission under both the average CSI scenario and the perfect CSI scenario.}}


